On the Detectability of ChatGPT Content: Benchmarking, Methodology, and Evaluation through the Lens of Academic Writing

With ChatGPT under the spotlight, utilizing large language models (LLMs) to assist academic writing has drawn a significant amount of debate in the community. In this paper, we aim to present a comprehensive study of the detectability of ChatGPT-generated content within the academic literature, particularly focusing on the abstracts of scientific papers, to offer holistic support for the future development of LLM applications and policies in academia. Specifically, we first present GPABench2, a benchmarking dataset of over 2.8 million comparative samples of human-written, GPT-written, GPT-completed, and GPT-polished abstracts of scientific writing in computer science, physics, and humanities and social sciences. Second, we explore the methodology for detecting ChatGPT content. We start by examining the unsatisfactory performance of existing ChatGPT detecting tools and the challenges faced by human evaluators (including more than 240 researchers or students). We then test the hand-crafted linguistic features models as a baseline and develop a deep neural framework named CheckGPT to better capture the subtle and deep semantic and linguistic patterns in ChatGPT written literature. Last, we conduct comprehensive experiments to validate the proposed CheckGPT framework in each benchmarking task over different disciplines. To evaluate the detectability of ChatGPT content, we conduct extensive experiments on the transferability, prompt engineering, and robustness of CheckGPT.

==> CheckGPT/tex/background.tex <==
\section{Related Work}
\label{sec:background}\label{sec:llm}\label{sec:related}

%\subsection{Large Language Models (LLMs)} \label{sec:llm}
% Language model, large-scale pre-training, large-size model and emergent ability\\
\noindent\textbf{Neural Language Models and LLM.} Neural networks for word probabilistic modeling have been developed since the 2000s \cite{bengio2000neural, sundermeyer2012lstm, cho2014learning}. Recently, pre-trained language models with general but effective word representation have been widely used, e.g., BERT \cite{devlin2018bert}, RoBERTa \cite{liu2019roberta}, ELMo \cite{emlo2018}, GPT-2 \cite{radford2019language}, and BART \cite{lewis2019bart}. The large language models (LLMs) are trained on massive amounts of data with deep learning frameworks consisting of an ultra-large amount of parameters. ChatGPT is built on top of OpenAI's GPT-3.5 with fine-tuning through supervised and reinforcement learning. %Benefited from the large-scale autoregressive pre-training based on transformer networks and comprehensive fine-tuning based on reinforcement learning from human feedback (RLHF), 
%ChatGPT is proven to mimic a versatile human conversationalist and succeed in many writing generation tasks, such as creating student essays, legal documents, business pitches, poetry/song lyrics, and programming codes.

% \begin{table*}[ht!]
%     \centering
%     \caption{Summary of SOTA LLM-content Detectors. Tool: used/evaluated online detection tools. Open: open-sourced.}
%     \vspace{-2mm}
%     \label{tab:literature}
%     \begin{footnotesize}
%     \setlength{\tabcolsep}{0.7em}
%     \begin{tabular}{|M{1.05cm}|M{0.6cm}||M{0.55cm}|M{0.8cm}|M{0.7cm}|M{0.85cm}||M{0.8cm}||M{1.2cm}||M{0.55cm}|M{0.55cm}|M{0.55cm}|M{1.0cm}||M{1cm}|M{0.55cm}|}
%         \hline
%         \multicolumn{2}{|c||}{\multirow{2}{*}{Study}} & \multicolumn{4}{c||}{Approach} &  \multirow{2}{*}{\parbox{0.8cm}{Transfer\\-ability}} & \# Human & \multicolumn{4}{c||}{Domain}  &  \multicolumn{2}{c|}{Dataset}   \\
%         \cline{3-6}\cline{9-14}
%          \multicolumn{2}{|c||}{}& Tool & Stat & Human & Train DNNs &&  Evaluators & News & QA & Essay & Research & Size & Open\\
%         \hline
        
%         \hline
%          \multirow{5}{*}{\parbox{1.2cm}{Grover or\\GPT-2\&3}} 
%         & \cite{gehrmann2019gltr} &
%           & \ding{108}& &            &
%           $-$ & $-$ & 
%           \ding{108}& & & \ding{108}           & 
%           $300$ &\\ 
%          \cline{2-14}
%          & \cite{kushnareva2021artificial} &
%           & \ding{108}& &  \ding{108}          &
%            $-$ & $-$ &
%           \ding{108}& & &            & 
%           $90k$ & \ding{108}\\ 
%           \cline{2-14}
       
%         & \cite{mitchell2023detectgpt} &
%           \ding{108}& & &            &
%            $-$ & $-$ &
%           \ding{108} & & \ding{108} &            & 
%           $-$ &\\
%           \cline{2-14}
%            & \cite{theocharopoulos2023detection} &
%           & \ding{108}& & \ding{108}           &
%            & $-$ &
%           & & & \ding{108}           & 
%           $28k$ & \ding{108} \\
%         \cline{2-14}
%          & \cite{zellers2019defending} &
%           & & \ding{108} &  \ding{108}          &
%            &  $*$ &
%           \ding{108} & & &            & 
%           $20k$ & \ding{108} \\ 
%          \hline
         
%          \hline
         
%          \multirow{8}{*}{ChatGPT} 
%             & \cite{bleuminkkeeping} &
%           & & & \ding{108}           &
%           & $-$ &
%           & & \ding{108} &            & 
%           $100k$&\\
%          \cline{2-14}
%          & \cite{gao2022comparing} &
%           \ding{108}& & \ding{108}&            &
%           $-$ & $2$ &
%           & & &  \ding{108}          & 
%           $100$&\\ 
%         \cline{2-14}
%         & \cite{guo2023close} &
%           & \ding{108}& \ding{108}&  \ding{108}          &
%           & $17$ &
%           & \ding{108} & &            & 
%           $125k$&\ding{108}\\
%           \cline{2-14}
%         % & \cite{he2023mgtbench} &
%         %   \ding{108}& \ding{108}& & \ding{108}           &
%         %   & \ding{108} & &            & 
%         %   $2817$\\
%         %  \cline{2-11}
        
%         & \cite{he2023mgtbench} &
%           \ding{108}& \ding{108}& & \ding{108}           & \ding{108}
%           & &
%           & \ding{108} & &            & 
%           $6k$&\ding{108}\\
%          \cline{2-14}

%          & \cite{kumari2023demasq} &
%           & \ding{108}& \ding{108} &            &
%            &  &
%            & \ding{108} &  &     \ding{108}       & 
%           $134k$& \\
%          \cline{2-14}
         
%          & \cite{liu2023argugpt} &
%           \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
%           & $43$ &
%           & & \ding{108} &            & 
%           $8k$&\ding{108}\\
%          \cline{2-14}

%          & \cite{macko2023multitude} &
%           \ding{108}& \ding{108}& & \ding{108}           &
%           & &
%          \ding{108} & &  &            & 
%           $74k$&\ding{108}\\
%          \cline{2-14}

%          & \cite{wang2023m4} &
%           & \ding{108}& & \ding{108}           &
%           \ding{108} &  &
%           \ding{108} & \ding{108} & \ding{108} &     \ding{108}       & 
%           $122k$&\ding{108}\\
%          \cline{2-14}

         
%          & Ours &
%           \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
%           \ding{108} & {\color{blue}{\textbf{155 + 87}}} &
%           \ding{108} & & \ding{108} &  \ding{108}          & 
%           {\color{blue}{\textbf{>2385k}}}&\ding{108}\\
%          \cline{2-14}
%          \hline

%          \hline
%     \end{tabular}\\
% % \vspace{-3mm}
% \begin{flushleft}
% $*$ The number of human evaluators is not explicitly provided.
% \end{flushleft}
% \vspace{-4mm}
% \end{footnotesize}
% \end{table*}

\begin{table}[t]
    \centering
    \caption{Summary of SOTA LLM-content Detectors.}% Tool: used/evaluated online detection tools. Open: open-sourced.}
    \vspace{-2mm}
    \label{tab:literature}
    \begin{footnotesize}
    \setlength{\tabcolsep}{0em}
    \begin{tabular}{|M{0.35cm}|M{0.6cm}||M{0.5cm}|M{0.45cm}|M{0.55cm}|M{0.55cm}||M{0.8cm}||M{0.7cm}||M{0.55cm}|M{0.45cm}|M{0.6cm}|M{0.5cm}||M{0.7cm}|M{0.6cm}|}
        \hline
        \multicolumn{2}{|c||}{\multirow{2}{*}{Study}} & \multicolumn{4}{c||}{Approach} &  \multirow{2}{*}{\parbox{0.8cm}{Transfer\\-ability}} & \#Hum. & \multicolumn{4}{c||}{Domain}  &  \multicolumn{2}{c|}{Dataset}   \\
        \cline{3-6}\cline{9-14}
         \multicolumn{2}{|c||}{}& Tool & Stat & Hum & DNN &&  Evalu. & News & QA & Essay & Res. & Size & Open\\
        \hline
        
        \hline
        % \parbox{1.2cm}{Grover or\\GPT-2\&3}
        %\multirow{5}{*}{\rotatebox[origin=c]{90}{\parbox{1cm}{Grover or\\GPT-2\&3}}}
        \multirow{5}{*}{\rotatebox[origin=c]{90}{Pre-ChatGPT}}
         %\multirow{5}{*}{\parbox{1.2cm}{Grover or\\GPT-2\&3}} 
        & \cite{gehrmann2019gltr} &
          & \ding{108}& &            &
          $-$ & $-$ & 
          \ding{108}& & & \ding{108}           & 
          $300$ &\\ 
         \cline{2-14}
         & \cite{kushnareva2021artificial} &
          & \ding{108}& &  \ding{108}          &
           $-$ & $-$ &
          \ding{108}& & &            & 
          $90k$ & \ding{108}\\ 
          \cline{2-14}
       
        & \cite{mitchell2023detectgpt} &
          \ding{108}& & &            &
           $-$ & $-$ &
          \ding{108} & & \ding{108} &            & 
          $-$ &\\
          \cline{2-14}
           & \cite{theocharopoulos2023detection} &
          & \ding{108}& & \ding{108}           &
           & $-$ &
          & & & \ding{108}           & 
          $28k$ & \ding{108} \\
        \cline{2-14}
         & \cite{zellers2019defending} &
          & & \ding{108} &  \ding{108}          &
           &  $^a$ &
          \ding{108} & & &            & 
          $20k$ & \ding{108} \\ 
         \hline
         
         \hline
         
         \multirow{9}{*}{\rotatebox[origin=c]{90}{ChatGPT}} 
            & \cite{bleuminkkeeping} &
          & & & \ding{108}           &
          & $-$ &
          & & \ding{108} &            & 
          $100k$&\\
         \cline{2-14}
         & \cite{gao2022comparing} &
          \ding{108}& & \ding{108}&            &
          $-$ & $2$ &
          & & &  \ding{108}          & 
          $100$&\\ 
        \cline{2-14}
        & \cite{guo2023close} &
          & \ding{108}& \ding{108}&  \ding{108}          &
          & $17$ &
          & \ding{108} & &            & 
          $125k$&\ding{108}\\
          \cline{2-14}
        % & \cite{he2023mgtbench} &
        %   \ding{108}& \ding{108}& & \ding{108}           &
        %   & \ding{108} & &            & 
        %   $2817$\\
        %  \cline{2-11}
        
        & \cite{he2023mgtbench} &
          \ding{108}& \ding{108}& & \ding{108}           & \ding{108}
          & &
          & \ding{108} & &            & 
          $6k$&\ding{108}\\
         \cline{2-14}

         & \cite{kumari2023demasq} &
           \ding{108} & \ding{108}& &            &
           &  &
           & \ding{108} &  &     \ding{108}       & 
          $134k$& \\
         \cline{2-14}
         
         & \cite{liu2023argugpt} &
          \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
          & $43$ &
          & & \ding{108} &            & 
          $8k$&\ding{108}\\
         \cline{2-14}

         & \cite{macko2023multitude} &
          \ding{108}& \ding{108}& & \ding{108}           &
          & &
         \ding{108} & &  &            & 
          $74k$&\ding{108}\\
         \cline{2-14}

         & \cite{wang2023m4} &
          & \ding{108}& & \ding{108}           &
          \ding{108} &  &
          \ding{108} & \ding{108} & \ding{108} &     \ding{108}       & 
          $122k$&\ding{108}\\
         \cline{2-14}

         
         & Ours &
          \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
          \ding{108} & {\color{blue}{\textbf{242$^b$}}} &
          \ding{108} & & \ding{108} &  \ding{108}          & 
          {\color{blue}{\textbf{>2.8m}}}&\ding{108}\\
         \cline{2-14}
         \hline

         \hline
    \end{tabular}\\
% \vspace{-3mm}
\begin{flushleft}
Pre-ChatGPT: Grover and GPT-2/3. Tool: used/evaluated online detection tools. Sat: Statistical approach. Hum: human evaluation. \# Hum. Evalu.: number of human evaluators. Res.: research papers/abstracts. Open: open-sourced.
\\$^a$ The number of human evaluators is not explicitly provided.
\\$^b$ 155 evaluators in the first experiment and 87 evaluators in the second experiment. 
\end{flushleft}
\vspace{-4mm}
\end{footnotesize}
\end{table}

\noindent\textbf{LLM-Content Detection.}  The detection of LLM-texts can be categorized into white-box and black-box approaches \cite{tang2023science}. %Black-box approaches are further categorized into feature-based and model-based detectors \cite{tang2023science}. 
Prior works \cite{gehrmann2019gltr, kushnareva2021artificial, mitchell2023detectgpt, theocharopoulos2023detection, zellers2019defending} study LLM-content detection for pre-ChatGPT models. \cite{gao2022comparing} evaluated 50 ChatGPT-written biomedical research abstracts with human reviewers and a RoBERTa-based classifier. Their findings show that 34\% of the abstracts are labeled as likely human-written. \cite{bleuminkkeeping} trained a transformer-based deep learning model to distinguish between AI-generated and human-written essays in a range of different education levels. \cite{guo2023close} and \cite{liu2023argugpt} conduct comprehensive studies, including human evaluators. \cite{guo2023close} analyzes a series of question-answering datasets in both English and Chinese, and \cite{liu2023argugpt} targets essays written by students and English learners. \cite{he2023mgtbench} establishes the first machine-generated text benchmark evaluating a number of detection approaches. 

The detailed comparisons of existing GPT detectors are listed in Table~\ref{tab:literature}. Compared with the other approaches, \checkgpt~(1) collects/uses a significantly larger dataset, (2) uses a model-agnostic design for higher affordability, upgradability, and flexibility, and (3) achieves very high accuracy, transferability, and interoperability. 

DEMASQ \cite{kumari2023demasq} is the most recent work that is similar to \checkgpt. It designed an energy-based model to identify the inherent differences between GPT- and human-generated text. Experiments across 8 sub-datasets achieved an accuracy of 73.9\% to 100\%. DEMASQ employs a very different attack model as it assumes alterations to ChatGPT output made by humans
to evade detection. Its detailed alteration algorithm, datasets, and models are not yet open-sourced, therefore, we are unable to run a comparative study. 

%We run our own sanitization methods on ChatGPT-generated data and demonstrate all the implementation details and results in 

\noindent\textbf{Security and Ethics in AIGC Application.} AI-generated content (AIGC) has been used in adversarial activities before LLMs were introduced \cite{ferrara2016rise}, while ChatGPT may provide a powerful tool to malicious actors \cite{renaud2023chatgpt,derner2023beyond}. The detection of AI-backed bots, scams, and misinformation has been extensively studied in the literature  \cite{cresci2020decade,shahid2022detecting,yang2020scalable,lu2022effects}, while the rise of ChatGPT introduces both new opportunities \cite{heidari2021bert,heidari2020using,dukic2020you,garcia2019empirical,hoes2023using,wang2023bot} and challenges \cite{gradonm2023electric,de2023chatgpt,mansfield2023weaponising,grbic2023social,roy2023generating,hazell2023large,cambiaso2023scamming}. While Open AI has enforced internal mechanisms to prohibit the unethical use of ChatGPT, the restrictions could be evaded \cite{li2023multi,liu2023jailbreaking}. Finally, there are also discussions and concerns with ChatGPT's potential impact on education and research \cite{stokel2022ai,willems2023chatgpt, firat2023chatgpt}, especially on authorship and plagiarism  \cite{stokelchatgpt,flanagin2023nonhuman,khalil2023will,anders2023using}.  %A small-scale experiment in \cite{gao2022comparing} showed that most of the GPT-generated abstracts were deemed as completely original by a web-based plagiarism detector (\url{https://plagiarismdetector.net/}).

%Most of the other methods use smaller datasets, except \cite{guo2023close}, which 



%Aiming at modeling the sequences of tokens in human-written texts as unprecedentedly sophisticated probability distributions, LLMs are capable of generating highly sophisticated language outputs that can achieve human-like language style and quality. The most notable examples of LLMs are the OpenAI GPT (Generative Pre-trained Transformer) series models, including ChatGPT, an advanced GPT-3 model trained on 175 billion parameters. One of the most prominent characteristics of LLMs is their significant rise in performance brought by the scaling effect, which can not be observed in small models. For example, work \cite{zhao2023survey} summarizes the emergent abilities of LLMs in three aspects: (1) in-context learning, (2) instruction following, and (3) step-by-step reasoning. In work \cite{wei2022emergent}, emergent abilities are validated in major LLMs (e.g., LaMDA \cite{thoppilan2022lamda}, GPT-3 \cite{brown2020language}, Gopher \cite{rae2021scaling}) through a series of few-shot prompted tasks \cite{brown2020language}, where the performance of accuracy jumps sharply from close-to-zero at under-$10^{22}$ FLOPs\footnote{Floating point operations per second (FLOPs) measures the scale of model parameters.} models to 40\% at $10^{23}$ FLOPs model.

% GPT3, transformer, RLHF training, excellent performance in many domain, concerns
%ChatGPT is built on top of OpenAI's GPT-3.5 with fine-tuning through both supervised and reinforcement learning techniques. Benefited from the large-scale autoregressive pre-training based on transformer networks and comprehensive fine-tuning based on reinforcement learning from human feedback (RLHF), ChatGPT is proven to mimic a versatile human conversationalist and succeed in many writing generation tasks, such as creating student essays, legal documents, business pitches, poetry/song lyrics, and programming codes.

%\subsection{Detection of LLM-Generated Texts}
% worries in academic integraty, 
%While the writing ability of LLMs has brought tremendous improvement in the efficiency for people's daily work, 
% The concern of LLM/ChatGPT misuse has been raised widely in academia because (1) academic integrity violations such as cheating and plagiarism will become {\em easy-to-conduct} and {\em hard-to-detect}. With the generative character of GPT, the texts for the same prompt can be very different at each time, but all can present human-like patterns and styles. %Whether having GPT to generate paragraphs based on a given topic or making GPT to polish existing paragraphs, t
% The GPT-generated outputs with effortless clicks are most likely to pass existing plagiarism checkers predefined by hand-craft rules (e.g., exact match scanning). (2) False and redundant information may flood the publication systems. Although ChatGPT is good at mimicking a human writer and showing plenty of details, the facts in its output can frequently be wrong, especially in STEM subjects. For example, %since the average rate of getting correct and factual answers from ChatGPT is too low, 
% Stack Overflow had to ban LLM-generated posts to ensure that visitors are able to find reliable answers efficiently \cite{stackoverflowbanchatgpt} %\footnote{https://meta.stackoverflow.com/questions/421831/temporary-policy-chatgpt-is-banned}. 
% With the same consideration, academic conferences started to ban LLM-generated texts (e.g., ICML). Rules are also enforced to clearly state LLM usages in acknowledgment (e.g., Nature and RSC).

% The detection of LLM-generated texts can be categorized into white-box and black-box approaches \cite{tang2023science}. Requiring full access to the target LLM, white-box approaches implant watermarks into LLM outputs and detect the watermarks to identify machine-generated texts. However, the owners of LLMs are increasingly reluctant to open-source their models, black-box approaches that only gather the output of LLMs have attracted more interest. They can be further categorized into (1) feature-based by examining hand-crafted statistical disparities, linguistic patterns, and fact verification \cite{tang2023science}; and (2) model-based by learning another language model, which is good at discriminating linguistic characteristics between human-written and machine-generated texts. Our approach falls into the second category. 

%As the size of LLMs is increasing by orders of magnitude (e.g., hundreds of billion parameters in GPT-3 comparing to trillions of parameters in GPT-4), white-box methods 

% \input{tex/related}

==> CheckGPT/tex/checkgpt.tex <==
\section{\checkgpt: An Accurate Detector for ChatGPT-generated Academic Writing}\label{sec:checkgpt}

\subsection{The System Model and Assumptions}\label{subsec:model}

%Our objective is to build a classifier, \checkgpt, to determine whether a given text is generated by ChatGPT. 
% We denote the \checkgpt~classifier as $\mathcal{H}$. The classification problem can be formulated as:
% \iffalse
% \begin{equation}
% % c=\underset{\{h, g\}}{\argmax {\:softmax(\mathcal{f}}(\mathbf{s}))
% y=\{y_{k}\}_{k\in \mathtt{C}}=\mathcal{H}(\mathbf{s})
% \end{equation}
% \begin{equation}
% c = \underset{k}{\argmax}\:y
% \end{equation}
% where $\mathbf{s}$ represents an unstructured text snippet (abstract). Given $\mathbf{s}$, $\mathcal{H}(\mathbf{s})$ outputs the probability distribution $y$ considering label space $\mathtt{C}=\{\text{`h'}, \text{`g'}\}$, where `h' indicates HUM-WRI and `g' indicates GPT-GEN. The predicted label $c$ can be derived accordingly.
% \fi

Our objective is to build a classifier, \checkgpt, to determine whether a given text snippet is generated by ChatGPT. We denote our classifier as $\mathcal{H}$, and the classification problem can be formulated as:

\vspace{-3mm}
\begin{equation}
% c=\underset{\{h, g\}}{\argmax {\:softmax(\mathcal{f}}(\mathbf{s}))
\hat{y}=\mathcal{H}_{\theta}(\mathbf{s})
\end{equation}
\begin{equation}
{\argmin}_\theta\:\mathcal{L}(y, \hat{y})
\end{equation}
where $\mathbf{s}$ is an unstructured text snippet (i.e., paper abstract). Given $\mathbf{s}$, $\mathcal{H}(\mathbf{s})$ generates the probability distribution $\hat{y}$ considering label space $\{\text{`h'}, \text{`g'}\}$, where `h' indicates human-written text and `g' indicates ChatGPT-generated text. The goal is to find an optimal set of parameter $\theta$ for $\mathcal{H}$ to minimize the loss function $\mathcal{L}$ measuring the distance between prediction $\hat{y}$ and observation ${y}$.
% We assume a \textit{black-box detector}, i.e., the detector could only observe samples that are known to be generated by ChatGPT or written by humans. The detector does not have any insider knowledge of the large language model, including the structure and the weights, in ChatGPT. All the datasets and off-the-shelf models we use in \checkgpt~are publicly available. 

We consider a \textit{black-box defender}, who only has access to the observed LLM outputs, and does not have insider knowledge of the LLM that generates these samples (weights, structures, and gradients). This assumption is practical, considering OpenAI has not open-sourced its LLMs since the GPT-3.5. %Thus, the defender's knowledge about the model of ChatGPT should be limited. 
%It is worth noting that all the models and datasets in \checkgpt~are publicly available. 

The primary goal of this work is to detect \textit{raw} ChatGPT-generated text, i.e., the unaltered output from ChatGPT. In the community, there have been discussions on the boundary between GPT-generated text and Human-generated text in the context of partial paraphrasing \cite{acl2023policy}, where the boundary can become murky if a piece of GPT-generated text is further edited by a human editor. Therefore, to avoid the controversy of data labeling, 
%we intentionally avoid the cases of ``what constitutes GPT-generated text?''. Instead, 
we mainly focus on the clean boundary between purely human-generated text and raw ChatGPT output in problem setting\footnote{We will relax this assumption in Section \ref{sec:robustness} and evaluate \checkgpt's robustness against \textit{post facto} human interventions}.%, including rephrasing, mixed human/GPT writing, and copyediting. 

%However, at the end of the paper, we will relax this assumption and demonstrate \checkgpt's robustness against \textit{post facto} human intervention, including rephrasing, mixed human/GPT writing, and copyediting (in Section \ref{sec:robustness}). However, we do not claim that \checkgpt~could stay effective after arbitrarily manual manipulation over the ChatGPT outputs. Indeed, we expect any detector, including \checkgpt, to degrade after increasing human intervention. 

Based on the application of the task, we further assume the following demands in addition to the defender's goals: (1) \textit{Moderate Data Availability}. We do not assume the defender's privileged usage of ChatGPT. Therefore, the training samples are collected strictly following OpenAI's policy. With the efficiency of regular queries, an ordinary user usually can not collect massive amounts (e.g., tens of millions to billions) of data. 
%Hence, the defender focuses on a more concise and domain-specific task.
(2) \textit{Affordability.} We do not assume the defender's access to excessive computing power, which is only affordable to large organizations in real world. We aim to offer a lightweight solution that smaller entities could conveniently obtain and deploy in a daily operational environment. And (3) \textit{Privacy-Preserving Local Deployment.} The end users may not agree to share their data with the detector providers due to privacy, intellectual property, or policy concerns (e.g., manuscripts being reviewed). Therefore, the detector should have the potential to be transferred to a new domain with a small amount of target-doman data. 

% We do not assume privileged access to ChatGPT or abusive use of ChatGPT. That is, we collect the training and testing samples as regular users. With the rate limit set by ChatGPT, a regular user cannot have millions or billions of training samples. In addition, we do not assume excessive computing power that is only affordable to large organizations. We attempt to develop a model that could be easily adopted by smaller entities. 

% \checkgpt~is a \textit{black-box detector}, which needs only the access to the observed samples, i.e., no insider knowledge of ChatGPT. We further make the following assumptions: (1) \textit{Moderate data} -- with the rate limit and cost of OpenAI's API, an ordinary user cannot have massive amounts (billions) of training samples. (2) \textit{Affordability} -- we develop a lightweight solution that smaller entities without requiring excessive computing power could easily adopt. And (3) \textit{Local deployment} -- the detector should be easily transferred to a new domain using a small amount of potentially private data from the target domain. 
% Finally, all the models and datasets used in \checkgpt~are publicly available. 


% \begin{itemize}[noitemsep, topsep=1mm, left=0pt]

% \item \textbf{Moderate Data Availability.} We do not assume the defender's privileged access to or abusive use of ChatGPT. The training and testing samples are collected strictly following OpenAI's policy. With the rate limit and pricing, an ordinary user cannot have massive amounts (tens of millions to billions) of samples. %For example, quantities in the millions or billions should be infeasible. 
% Hence, the defender focuses on a more concise and domain-specific task. 

% \item \textbf{Affordability.} We do not assume the defender's access to excessive computing power, which is only affordable to large organizations. We aim to develop a lightweight solution that smaller entities could conveniently obtain and deploy in a daily operational environment. 

% \item \textbf{Privacy-preserving Local Deployment.} The end users may not want to share their data with a detection service provider due to a variety of concerns, such as privacy, intellectual property, or policy, e.g., student essays or papers under review. Therefore, the detector should be easily transferred to a new domain using a small amount of data from the target domain and affordable computation resources. 
% \end{itemize}

% \subsection{The Baseline Approaches}\label{subsec:baseline}

% In the baseline approaches, we employ TF-IDF for document representation and then use PCA to reduce the feature space to 100 dimensions. We adopt three non-deep-learning models to classify HUM and GPT-GEN abstracts: Gaussian Naive Bayes (GNB), SVM, and random forest (RF). We use a 70/30 train-test split ratio on 100,000 samples (50,000 HUM and 50,000 GPT from Prompt 1) for each task and discipline. %Each model is trained and evaluated under the same conditions.

% The performance of the baseline models is shown in Table \ref{tab:baseline}. We have the following observations: (1) While NB has been widely used in text analysis~\cite{mitchell2007machine, sahami1998bayesian}, it performs poorly across all the tasks. This indicates that the assumptions (e.g., Gaussian Distribution and Independence) may not hold in this problem. (2) For Task 1, SVM and RF perform well in distinguishing GPT-written abstracts in CS and physics. However, their performance decreases to approximately 80\% for HSS. A possible explanation is that the abstracts fully written by ChatGPT demonstrate \textit{unique lexical features} that are easily distinguishable with linear classifiers. (3) For Task 2, the accuracy of SVM and RF drops to 86\% for Computer Science, 90\% for Physics, and around 70 \% for humanity and social sciences. (4) The GPT-polished abstracts in Task 3 are more challenging to detect. The performance of the SVM and RF decreases sharply to 52\% and 58\% for CS and HSS, respectively, and to 70\% for physics. 

% %\item Across all three classifiers, physics appears to be the easiest for classification. Abstracts in Humanity and Social Sciences present the most difficulty.

% % \begin{itemize}[noitemsep, topsep=1mm, left=0pt]
% % \item The Naive Bayes classifier, which has been widely used in text analysis~\cite{mitchell2007machine, sahami1998bayesian}, performs poorly across all the tasks. This indicates that the assumptions (e.g., Gaussian Distribution and Independence) may not hold in this problem.

% % \item For Task 1, SVM and Random Forest perform well in distinguishing GPT-written abstracts in CS and physics. However, their performance decreases to approximately 80\% for HSS. A possible explanation is that the abstracts fully written by ChatGPT demonstrate \textit{unique lexical features} that are distinguishable with linear classifiers.

% % \item For Task 2, the accuracy of SVM and Random Forest drops to 86\% for Computer Science, 90\% for Physics, and around 70 \% for humanity and social sciences.

% % \item The GPT-polished abstracts in Task 3 are more challenging to detect. The performance of the SVM and Random Forest decreases sharply to 52\% and 58\% for CS and HSS, respectively, and to 70\% for physics. 

% % %\item Across all three classifiers, physics appears to be the easiest for classification. Abstracts in Humanity and Social Sciences present the most difficulty.
% % \end{itemize}

% In summary, while the baseline approach lacks capabilities in some tasks, it still significantly outperforms human evaluators in Section \ref{sec:survey}. As the TF-IDF model only captures the lexical features, the success of SVM and RF in Task 1 implies that ChatGPT writes with different term distributions than humans, especially in physics, where human authors may use more math/technical terms than ChatGPT. However, the detection accuracy decreases significantly in Task 3, implying that GPT-polished abstracts tend to adopt the vocabulary and term distribution from the seed human-written abstracts. 

%However, their practical utilities are limited in real-world applications, as they are unable to deal with complex scenarios, especially when subtle or moderate changes are applied.

% In the baseline approach, we utilize the vector space (tf-idf) model for text representation and then employ a classifier for human-GPT classification. Three non-DL classifiers are adopted: Gaussian naive Bayes (GND), support vector machine (SVM), and random forest (RF). 
% Each model is trained with 35,000 samples from each class (human vs. GPT), and tested with 15,000 samples from each class, i.e., a 0.7/0.3 train-test split ratio. The overall classification accuracy of each model on each task and dataset is demonstrated in Table \ref{tab:baseline}. We have the following observations from the results: (1) The Gaussian naive Bayes model performs poorly on all tasks. (2) SVM and random forest both provide solid performance in distinguishing GPT-generated full abstracts in CS and physics (accuracy > 96\%). However, the performance decreases to ~80\% for humanity and social sciences. (3) For the GPT-completed abstracts in Task 2, the classification accuracy of SVM and RF decreases to 86\% for CS, 90\% for physics, and ~70\% for HSS. (4) The GPT-polished abstracts in Task 3 appear to be very difficult to detect, as the classification accuracy  further decrease to 52\% to 58\% for CS and HSS, and ~74\% for physics. (5) disciplines. In summary, the baseline classifiers perform better than human users (compared with the user study results in Section \ref{sec:survey}). However, not practical...

% \begin{table}[t]
% 	\caption{The baseline approach: accuracy (in \%) for each classifier on each task and each discipline dataset.}\label{tab:baseline}
%     \setlength{\tabcolsep}{0.2em}
%     \centering

%     \vspace{-2mm}
%     {\small
% 	\begin{tabular}{c|ccc|ccc|ccc}
%       \multirow{2}{*}{Model} & \multicolumn{3}{c|}{T1. GPT-WRI} &\multicolumn{3}{c|}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\
% 		\cline{2-10}
%         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
% % GNB	& 53.3	&	51.9	&	52.2	&	52.1	&	51.7	&	50.8	&	50.2	&	50.5	&	51.4	\\
% % SVM	& 96.4	&	98.2	&	74.8	&	86.4	&	90.5	&	66.5	&	57.8	&	75.9	&	53.3	\\
% % RF	& 96.5	&	98.2	&	84.8	&	87.4	&	90.5	&	72.9	&	52.0	&	72.7	&	58.7	\\
% GNB	& 95.0	&	98.1	&	94.1	&	91.4	&	95.5	&	90.2	&	82.1	&	90.0	&	71.8	\\
% SVM	& 98.3	&	99.1	&	97.5	&	96.5	&	96.8	&	94.9	&	92.1	&	93.9	&	89.4	\\
% RF	& 99.0	&	99.8	&	99.1	&	95.3	&	96.4	&	94.5	&	92.1	&	95.0	&	89.2	\\
%         \end{tabular}\vspace{-4mm}}
% \end{table}

\subsection{Linguistic \& Semantic-Based Detection}\label{subsec:baseline}
{
We first explore a non-deep learning method using hand-crafted linguistic \& semantic features as our baseline approach. The raw texts are transformed into vector representations using the NELA (News Landscape) features \cite{nela}. The NELA features were initially proposed to analyze news articles. They comprise six linguistic and semantic features: styles, complexity, biases, affects, morals, and events. We adopt Gradient Boosting (GB) decision trees to distinguish between human-written and GPT-generated abstracts. For each task and discipline, the models are trained with 50,000 human-written and GPT-generated samples, respectively, and tested with 10,000 samples from each class, i.e., an 80/20 train-test split ratio. %Each model is trained and evaluated under the same conditions.

The classification performance of the baseline models is shown in Table \ref{tab:baseline}. We have the following observations: (1) For Task 1, GB performs well in distinguishing GPT-written abstracts in CS and physics. (2) For Task 2, the F1-scores drop to about 0.9, indicating an increased difficulty. (4) The GPT-polished abstracts in Task 3 are more challenging to detect. The performance decreases significantly to <0.8 for all the three disciplines. 

We inspect the feature importance within GB model to analyze the difference between the GPT-generated and human-written abstracts. In general, we find that ChatGPT composes differently in several characteristics: (1) ChatGPT tends to compose longer sentences and use longer words during writing; (2) ChatGPT habitually uses more gerunds as adverbials; (3) ChatGPT uses more determiners, more gerunds, and fewer personal pronouns than human writers.
More details can be found in Appendix~\ref{apdx:nelagb}.

% ----- this part has been moved into appendix
%For Task 1, readability (Coleman-Liau Index \cite{colemanindex}) is always the dominating feature, regardless of the discipline. For example, the average Coleman-Liau index for computer science is 20.63 for GPT-WRI abstracts and 15.44 for HUM abstracts. This shows that ChatGPT tends to compose longer sentences and use longer words during writing, which makes the text harder to comprehend than human writing. 
%For Task 2, Coleman-Liau's readability is still the most important feature for all three disciplines, and its importance is far larger than the others. Other contributing factors include the gerunds or present verbs (for all three disciplines), Lix readability (for CS and PHX), possessive pronouns (for PHX), and Flesch–Kincaid readability (for HSS). For PHX, the average number of possessive pronouns is 0.05 for HUM abstracts, 0.18 for GPT-WRI abstracts, and 0.15 for GPT-CPL abstracts. Considering gerund or present verbs, the average numbers are 0.025, 0.017, and 0.024 for HUM abstracts in CS, PHX, and HSS, and these numbers nearly double for GPT-CPL abstracts. A possible explanation is that ChatGPT habitually uses more gerunds as adverbials. 
%For Task 3, the importance is more scattered among features. Readability and determiners are important across three disciplines. Gerunds and personal pronouns are important for CS and PHX. Specifically, ChatGPT uses more determiners, more gerunds, and fewer personal pronouns than human writers after polishing. Additionally, ChatGPT uses fewer non-third-person singular present verbs for PHX and HSS and more third-person singular present verbs for CS. 
%However, readability is consistently the most important feature, and most other differences (except gerunds) are subtle. Some of the patterns are unique and not general across disciplines or tasks, e.g., third-person singular present verbs. This explains the performance drop of the classifiers on Task 3.



%\noindent \textbf{{\em Takeaways.}} 
While the baseline approach lacks capabilities in some tasks, it still significantly outperforms the human evaluators tested in Section~\ref{sec:survey}, and the existing detecting tools in 
Table~\ref{tab:otherdetectors}. It showcases the different habitual patterns of GPT-generated and human-written abstracts. Prominently, ChatGPT exhibits a tendency of increased complexity and a higher frequency of third-person singulars and gerunds. While these habitual patterns identified provide valuable insights, they alone cannot guarantee reliable and generalizable classification, as shown by the model's insufficiency on Task 2 and 3. This motivates us to adopt DNN-based detectors, which are more capable of capturing subtler and deeper semantic and/or linguistic patterns that the hand-crafted NELA features may overlook.

\begin{table}[t]
	\caption{The baseline approach: classification F1-score for NELA classifier.}\label{tab:baseline}\vspace{-3mm}
    %\setlength{\tabcolsep}{0.2em}
    \centering
    {\small 
	\begin{tabular}{ccc|ccc|ccc}
     \multicolumn{3}{c|}{T1. GPT-WRI} &\multicolumn{3}{c|}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\ \hline
        CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
0.965	&	0.980	&	0.963	&	
0.901	&	0.918	&	0.896	&	
0.774	&	0.794	&	0.798	\\
        \end{tabular}
        }\vspace{-3mm}
\end{table}

}

\subsection{The CheckGPT Framework}
\noindent\textbf{{\em Preliminaries.}} The Bidirectional Encoder Representations from Transformers (BERT) \cite{devlin2018bert} family, including but not limited to BERT itself and RoBERTa, have shown extraordinary capabilities in a wide range of NLP tasks. RoBERTa (Robustly Optimized BERT approach) \cite{liu2019roberta}, is the state-of-the-art member of this family built upon BERT by Meta. Models like RoBERTa are pre-trained on a massive corpus from diverse disciplines. Such extensive training allows them to capture and represent various linguistic patterns, syntactic structures, and semantic relationships in the texts. Its tokenization and encoding enable the transformation of raw data into effective representations, which can be used for downstream tasks. In this work, we utilize the pre-trained RoBERTa to preprocess the text data. The pre-training of the RoBERTa utilizes a masked language modeling (MLM) objective, which can be formalized as:

\begin{equation}
\mathcal{L}_{\text{MLM}}=-\mathbb{E}_{\mathbf{s} \sim \mathcal{D}_{s}}{\log P(m | \mathbf{s})}
\end{equation}
\noindent where $\mathcal{D}_{s}$ is the corpus, $\mathbf{s}$ denotes an input sequence, and $m$ is a masked token. The representations extracted by RoBERTa serve as the features for our downstream classification head. Long-Short-Term Memory (LSTM) networks \cite{hochreiter1997long}, a variant of Recurrent Neural Network (RNN) which incorporates gating mechanism to effectively retain information, can improves feature extraction over long sequences. In this work, we adopt LSTM to build the classification head to aggregate the sequences of RoBERTa encoded tokens, and to fine-tune the final representation for task-specific prediction.

% LSTM and GRU are variants of RNN that have gained incredible success in natural language processing by handling sequential information. LSTM mitigates the gradient vanishing problem and improves model performance over long sequences by incorporating the gating mechanism, which enables it to effectively and selectively retain or update information. GRUs are similar to LSTMs but simpler and more efficient in terms of computation, which has two gates (update and reset gates) and no separate cell state.

\noindent\textbf{{\em Representation.}} 
\checkgpt~ framework consists of two stages: representation and classification, as shown in Figure \ref{fig:checkgpt}.
For representation, \checkgpt~proposes a model-agnostic design for text encoding where any pre-trained representation models (e.g., other variants of BERT) are directly employed as is. This design achieves higher affordability, upgradability, and flexibility since 
(1) adopting a sophisticated pre-trained embedding model can saves tremendous efforts and computations compared with training an embedding layer from scratch, which is often beyond the capability of regular users or organizations;
(2) a plugin design allows future upgrades by seamlessly accommodating new representation models; 
and 
(3) the lightweight classification head is easier to fine-tune when new data or domains are added.
In \checkgpt, the representation stage is completed using the tokenizer and encoders of RoBERTa-large\footnote{https://github.com/facebookresearch/fairseq/tree/main/examples/roberta}. For tokenization, the pre-trained RoBERTa-large enforces a limit of 512 tokens. The tokenization can be formalized as:
\begin{equation}
\mathbf{X} = \text{Tokenizer}(\mathbf{s}) = \{x_{i}\}_{i=1}^{n}
\end{equation}
\noindent where $\mathbf{X}$ denotes a sequence of length $n$ consisting of individual tokens $x_{i}$, and $\text{Tokenizer}$ refers to the Byte-level Pairing Encoding (BPE) utilized by RoBERTa.

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{CheckGPT/img/arch.png} %\vspace{-5mm}
\caption{The architecture of the \checkgpt~model.} %\vspace{-3mm}
\label{fig:checkgpt}\vspace{-3mm}
\end{figure}

For the encoder, the RoBERTa uses embeddings of size 1024 to represent each token. In this way, the tokenized texts are encoded into contextualized representations with a shape of $n \times 1024$. The encoding can be formalized as:
\begin{equation}
\mathbf{E} = \text{Encoder}(\mathbf{X}) = \{e_{i}\}_{i=1}^{n},\;\;   e_{i} \in \mathbb{R}^{1024} 
\end{equation}
\noindent where $\mathbf{E}$ denotes a sequence consisting of individual embedding $e_{i}$, and $\text{Encoder}$ refers to the transformer encoder utilized in RoBERTa.
% Our \checkgpt~ includes two stages: \textit{representation} and \textit{classification}. 
% For text representation, \checkgpt~adopts a model-agnostic design offering high affordability, upgradability, and flexibility.
%so that any tokenization and embedding model could be employed in this framework. This design achieves higher affordability, upgradability, and flexibility since 
% (1) adopting standardized and powerful embedding models saves lots of effort and computations compared with training a large embedding model, which is usually beyond the capability of regular users or organizations;
% (2) a plugin design allows future upgrades by seamlessly accommodating new representation models; and 
% (3) the lightweight classification head is easier to be tuned when new data or domains are added. 
% In our proof-of-concept prototype of \checkgpt, 
% the first stage is completed using the tokenizer and encoders of RoBERTa-large\footnote{https://github.com/facebookresearch/fairseq}\cite{liu2019roberta}. 
% Our proof-of-concept prototype of \checkgpt~uses the tokenizer and encoders of RoBERTa-large \cite{liu2019roberta}.
% % For tokenization, the pre-trained RoBERTa-large enforces a limit of 512 tokens. 
% The tokenization can be formalized as:

% \vspace{-3mm}
% \begin{equation}
% \mathbf{X} = \text{BPE}(\mathbf{s}) = \{x_{i}\}_{i=1}^{n}
% \end{equation}
% \vspace{-5mm}

% \noindent where $\mathbf{X}$ denotes a sequence of length $n$ consisting of individual tokens $x_{i}$, and $\text{BPE}$ refers to the byte-level pairing encoding utilized by RoBERTa.

% For the embedding layer, RoBERTa generates an embedding $e_{i}$ of size 1024 per token. The text sequences are transformed into contextualized representations $\mathbf{E}$ with a $n \times 1024$ shape. The encoding can be formalized as:
% \begin{equation}
% % \begin{split}
% \mathbf{E} = \text{TransformerEncoder}(\mathbf{X}) = \{e_{i}\}_{i=1}^{n}
% % ,\;\;   
% % \\ e_{i} \in \mathbb{R}^{1024} 
% % \end{split}
% \end{equation}
% \noindent where $\mathbf{E}$ denotes a sequence consisting of individual embedding $e_{i}$. 

\noindent\textbf{{\em Classification.}} The derived embeddings are fed into the LSTM-based classification stage. The classification head consists of two LSTMs (with embedding size of 256), and each has a following attention layer \cite{baziotis-etal-2018-ntua-slp-semeval} to aggregate the entire sequence into a single vector. The outputs from the two LSTMs modules are later concatenated and passed through a dropout layer with a rate of $p=0.5$ for overfitting prevention, and a dense layer (FC) for final task-specific fine-tuning. 
% The dense layer gives two output values. Each softmaxed output value represents the probability of belonging to each of the two classes: 
The softmaxed output indicates the conditional probability of the two classes: ``GPT-generated'' ($y_{g}$) or ``Human-generated'' ($y_{h}$). The functions of our LSTM classifier $f_{\theta}(\mathbf{E})$ are as follows:
\begin{equation}
\begin{aligned}
h_{1} = \text{LSTM}_{1}(\mathbf{E}),\;\;r_{1} = \text{ATTN}_{1}(h_{1}) \\
h_{2} = \text{LSTM}_{2}(h_{1}),\;\;r_{2} = \text{ATTN}_{2}(h_{2}) \\
(\hat{y}_{g}, \hat{y}_{h}) = \text{Softmax}(\text{FC}(\text{Dropout}(r_{1} \oplus r_{2})))
\end{aligned}
\end{equation}
\noindent\textbf{{\em Model Training.}} The classifier $f_{\theta}$ with parameter $\theta$ is optimized independently with the RoBERTa frozen (as is) during the training. We adopt an AdamW optimizer \cite{loshchilovdecoupled}, a CosineAnnealing learning rate scheduler \cite{loshchilovsgdr}, and a gradient scaler for efficient mixed-precision training \cite{micikeviciusmixed}. 
% We employ cross-entropy loss for binary classification. 
Given the model's predicted probabilities $\hat{y}=(\hat{y}_{h}, \hat{y}_{c})$ and one-hot encoded ground truth $y=(y_{h}, y_{c})$
, the Binary Cross Entropy (BCE) loss of each training sample is defined as: 
\iffalse
\begin{equation}
\mathcal{L}(\theta)=-\mathbb{E}_{(\mathbf{E},\hat{c}) \sim \mathcal{D}_{E}}\left[\hat{c} \log(f_{\theta}(\mathbf{E})) + (1-\hat{c}) \log(1 - f_{\theta}(\mathbf{E})\right]
\end{equation}
\fi
\begin{equation}
\mathcal{L}(\theta)=-\left[y_{c} \log(\hat{y}_{c}) + y_h \log(\hat{y}_{h})\right]
\end{equation}

% Plot overview, flops, equivals to gpu hours
\noindent\textbf{{\em Design Choices and Discussions.}} One alternative approach is directly applying RoBERTa by adding a RobertaClassificationHead \cite{robertahuggingface}. However, experiments show that \checkgpt~incur a higher accuracy, which can be attributed to LSTM's capability to track the sequential dependencies over long periods in the text sequences \cite{yin2017comparative}. Please refer to Section~\ref{sec:baselineperf} for details of the ablation study.

% We've tried other architectures like CNNs and MLPs, and found LSTM performs the best. 

Another alternative approach is to include the entire pre-trained language representation model \cite{ott2019fairseq, robertacustom} for task-specific fine-tuning. As shown in Table \ref{tab:opensourcedetector}, \checkgpt~ consistently outperforms the approaches of fine-tuning the entire language representation models (BERT, DistillBERT, RoBERTa, and GPT-2) on GPABench2.
% , i.e., the model adopts the pre-trained parameters as a warm start and gets retrained on the new dataset. 
%However, the training process requires much higher computing power and time. 
%Through weighing the cost and benefit, our \checkgpt~design has distinct advantages: 

Comparing with both alternative approaches in framework design, \checkgpt~ offers the following advantages: 
(1) \textbf{Efficiency}: \checkgpt~can significantly reduce the parameters to save both time and computing resources. Given the parameters of language models ranging from 66M (DistilledBERT \cite{sanh2019distilbert}) to 355M (RoBERTa-large, GPT-2-medium) and 1750M (GPT-3 \cite{brown2020language}), our model only maintain 4M parameters and achieve satisfactory accuracy. The drop in model size also reduces the risks of over-fitting and catastrophic forgetting \cite{mosbach2021stability, kirkpatrick2017overcoming}, especially with small datasets \cite{uchendu2020authorship, bakhtin2019real}.
(2) \textbf{Applicability}: Our framework is model-agnostic thus accepts various representation approaches (e.g., BERT\cite{devlin2018bert}, BART \cite{lewis2019bart}), making it a lightweight and universal detector, as detailed in Section~\ref{sec:baselineperf}.
% and can be used with almost any publicly available pre-trained language models. 
This feature can especially valuable considering deployment and customization in real world.
%. Explicit training for machine-generated text classification is known to suffer from overfitting to a specific domain\cite{uchendu2020authorship, bakhtin2019real}. 
(3) \textbf{Versatility}: By freezing RoBERTa's well-crafted parameters trained on a broad range of domains, we retain the framework's generalizability to a great extent to use \checkgpt~ in different subjects, which is challenging for fine-tuned RoBERTa \cite{wang2023m4}. More details are presented in Section~\ref{sec:transfer}.

%{\newc As shown in Table \ref{tab:opensourcedetector}, \checkgpt~consistently outperforms fine-tuning the entire Language Models (BERT, DistillBERT, RoBERTa, and GPT-2) on GPABench2. Furthermore, we will show that the performance of \checkgpt~is better on other state-of-the-art datasets in other domains in Section \ref{subsec:newdomain}.}


==> CheckGPT/tex/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

In this paper, we first present GPABench2, a benchmarking dataset with 2.385 million samples of human-written, GPT-written, GPT-completed, and GPT-polished research paper abstracts. Next, we show that the existing ChatGPT detectors and human users are incapable of identifying GPT-content in GPABench2. We further present \checkgpt, a deep learning-based detector for GPT-generated academic writing. With extensive experiments, we show that \checkgpt~is highly accurate, affordable, flexible, and transferable. 


==> CheckGPT/tex/datacollection.tex <==
\section{GPABenchmark: \underline{G}PT Cor\underline{p}us for \underline{A}cademia}\label{sec:gpabenchmark}


\subsection{The GPABench2 Dataset}\label{sec:subsecgpabenchmark}

The concern of LLM/ChatGPT misuse has been raised widely in academia because (1) academic integrity violations such as cheating and plagiarism will become {\em easy-to-conduct} and {\em hard-to-detect}. (2) False and redundant information may flood the publication systems. Stack Overflow had to ban LLM-generated posts to ensure that visitors can find reliable answers efficiently \cite{stackoverflowbanchatgpt} Academic conferences started to ban LLM-generated texts (e.g., ICML) or require disclosure (e.g., ACL, Nature, and  RSC). However, without effective mechanisms to detect GPT-generated content and benchmarking datasets to train/evaluate the detectors, such discussions and policies become meaningless. %Especially, our user study in Section \ref{sec:survey} shows that 

The state-of-the-art corpora for ChatGPT text classification mainly focus on question-and-answer (Q\&A) dialogues \cite{he2023mgtbench, guo2023close}. %because ChatGPT is intended to generate human-like conversational dialogues. 
While the Q\&A datasets align with the original design of ChatGPT as an interactive ``Chat'' interface, they become insufficient as the usage scenarios of ChatGPT have significantly expanded beyond chat.   %In particular, it has been reported that ChatGPT has been utilized 
When ChatGPT is adopted for academic writing, such as essays, reports, and even research papers \cite{firat2023chatgpt,stokel2022ai}, the generated text akin to academic writing style is often objective, formal, and focused \cite{guo2023close, liu2023argugpt}, posing more challenges to the detectors: (1) Human conversations often contain subjective opinions, personal biases, and emotions. However, such clues are significantly less observed in academic writing, which is generally formal and objective \cite{hyland2005stance, biber1991variation, biber2010challenging, guo2023close}. (2) Grammatical errors and inconsistencies in human-generated texts may serve as meaningful indicators, however, they are less likely to occur in academic writing, which is expected to meet higher standards for fluency, clarity, and grammatical correctness \cite{hinkel2003teaching, lynch2013grammar}.  Also, academic writers typically adopt a comprehensive and organized style \cite{cargill2021writing} akin to the one generated by ChatGPT \cite{guo2023close}. (3) Academic abstracts typically explore domain-specific and highly-specialized topics \cite{hyland2005stance}, which lead to a significantly different term distribution from conversational dialogues. 

With the unique characteristics of academic writing, a new ChatGPT-generated corpus is necessary for benchmarking GPT detectors and assisting in the design of detectors. 
In this paper, we introduce \textit{GPABench2} (GPABenchmark version 2), a large-scale \underline{G}PT-generated text cor\underline{p}us for \underline{a}cademic writing. 

We first collected research papers (title and abstracts) from three disciplines: \textit{computer science} (CS) abstracts from top-tier conference proceedings and arXiv, \textit{physics} (PHX) from arXiv, and \textit{humanities and social sciences} (HSS) from Springer's SSRN including history, philosophy, sociology, and psychology disciplines. The three fields spread across ``hard science'' (math-intensive) and ``soft science'' disciplines. For CS and Physics, we chose papers published or posted on or before 2019 (before the release of GPT-3) to ensure
that they were all human-written, as researchers may have adopted GPT-3 to assist their writings before the web-based ChatGPT was released\footnote{GPT-3 was first released in 06/2020, access to the test release was by-invitation-only until 11/2021 when the API was made publicly accessible.}. %For each paper, we store an identifier (ID), a title (T), and an abstract (ABS). 
Eventually, we collected 50,000 papers from each discipline. 

%For each paper, we recorded its ID, title (T), and abstract (ABS).

We define three tasks based on the most representative scenarios where LLMs are used/misused in academic writing: %users provide a title for text generation, provide a partial draft for completion, or provide a draft for polishing. %Hence, we define three different tasks where the users provide different amounts of information to ChatGPT:

\begin{itemize}[noitemsep, topsep=1mm, left=0pt]
\item\textbf{Task 1. GPT-written full abstracts (GPT-WRI or WRI).} The author gives a title to ChatGPT and asks it to write the complete abstract from scratch. 

%A sample prompt is: \textit{Please generate an abstract for a research paper titled ``Attitude of the Society Towards People with Visual Impairment.''}  

\item\textbf{Task 2. GPT-completed abstracts (GPT-CPL or CPL).} Text completion is considered a conventional function of LLMs: The author provides a few sentences to ChatGPT, who follows the logic to complete the rest of the paragraph. We mimic this scenario: for an abstract with $s$ sentences, the first $s/2$ sentences are provided to ChatGPT, based on which it \textit{completes the abstract with $w$ words}, where $w$ is the word count in the second half of the original abstract. Hence, the GPT-CPL abstract will have \textit{approximately} the same length as the human-written abstract. 

\item\textbf{Task 3. GPT-polished abstracts (GPT-POL or POL).} We provide the entire abstract to ChatGPT for polishing. %We adopt a popular prompt from the ChatGPT users' community: ``\textit{This is an abstract of a research paper. Please rewrite for clarity.}'' 
ChatGPT re-writes the text sentence-by-sentence and generates a revised abstract. Invoking ChatGPT multiple times will generate different results for the same seed abstract. 
\end{itemize}

% We define three tasks based on the most representative scenarios where LLMs are used or misused in academic writing. In {\em \textbf{Task 1: GPT-written full abstracts (GPT-WRI)}}, ChatGPT generates an abstract with only a given title. In {\em \textbf{Task 2: GPT-completed abstracts (GPT-CPL)}}, with some user-provided seed text, ChatGPT completes the rest of the essay following the logic of the seed. We mimic this scenario: for an abstract with $s$ sentences, the first $s/2$ sentences are provided to ChatGPT, based on which it \textit{completes the abstract with $w$ words}, where $w$ is the word count in the second half of the original abstract. In {\em \textbf{Task 3: GPT-polished abstracts (GPT-POL)}}, the entire abstract is provided to ChatGPT, which re-writes the text sentence-by-sentence.  %Invoking ChatGPT multiple times will generate different results for the same seed. 

% In the rest of the paper, we denote the abstracts written by human authors and ChatGPT as \textit{human-written} abstracts (HUM) and \textit{GPT-Generated} abstract (GPT-GEN), respectively. The latter is a superset of GPT-WRI, -CPL, and -POL.
In this paper, we use \textit{human-written} abstracts (HUM) to denote abstracts that are completely written by human authors. We use \textit{GPT-Generated} abstract (GPT-GEN) to denote all three categories of GPT-content described above: GPT-WRI, -CPL, and -POL. 
 

We applied prompt engineering in data collection to ensure a broad coverage of ChatGPT use cases. %To ensure that our data covers a broad range of use cases with diverse prompts, 
We studied popular prompt patterns \cite{white2023prompt} and prompt guidelines \cite{PlexPt2023prompt, Akın2023prompt, amiri2023prompt, jaiswal2023prompts} in the literature and crafted four distinct prompts for each task, denoted as Prompts 1 to 4 (presented in Appendix~\ref{apdx:prompt3}): Prompt 1 is a popular but straightforward zero-shot prompt. Prompt 2 integrates the contexts to outline the scope of a specific discipline. Prompt 3 uses the role-playing technique to specify a ``persona'', e.g., ``an expert paper writer in computer science''. Prompt 4 provides detailed requirements and instructions to guide ChatGPT. These prompts represent four use cases with increasing levels of knowledge fed to ChatGPT. 

We invoke ChatGPT (gpt-3.5-turbo) through OpenAI's API to generate abstracts at the cost of 0.2 cents per 1,000 tokens. In three months, we collected 50,000 samples for each prompt, task, and discipline, as the GPABench2 Main Dataset (1.8 million total GPT-GEN samples). We further adopted ten advanced prompting techniques, e.g., chain-of-thought and in-context prompt learning, to generate 435K additional testing samples (Sec. \ref{sec:discussion}). Eventually, GPABench2 contains 2.385M total samples (2.235M GPT-GEN and 0.15M HUM).

\vspace{2mm}\noindent\textbf{Advanced Prompt Engineering and Additional Testing Data.} Research efforts on prompt engineering aim to guide or improve the design of ChatGPT prompts \cite{white2023prompt,ekin2023prompt}. We adopt six approaches that are widely adopted in the community: (1) Zero-shot Chain-of-Thought Prompting (ZC, \cite{zeroshot}) enforces step-by-step reasoning with specific trigger phrases like ``Let's think step by step.'' (2) Automatic Prompt Engineer (APE, \cite{ape}) automates the creation and selection of prompts using iterative optimization. (3) Self-critique Prompting (SCP, \cite{critique}) employs GPT to evaluate its own responses and provide feedback. (4) Few-shot Prompting (FSP, \cite{fewshot}) conditions the model using examples or demonstrations. (5) Least-to-Most Prompting (LMP, \cite{least}) parses a problem into simpler subproblems. (6) Generated Knowledge Prompting (GKP, \cite{generated}) starts the prompt with relevant information generation. We also adopt four prompt refinement methods: (1) Prompt Perfect (PP, \cite{promptperfect}). (2) GPT-generated Prompts (GP, \cite{Creator}). (3) Meta Prompts (MP, \cite{metaprompt}). (4) Instruction Induction (II, \cite{honovich2022instruction}, not for Task 3). We use each method to write, complete, and polish 5,000 abstracts from each discipline (please refer to Appendix~\ref{apdx:otherprompt} for details). In summary, we collected 435K additional samples to be used for testing. 


%The GPABenchmark dataset with 600,000 samples is shared at: \url{https://github.com/GPABenchmark}. 

% \begin{figure*}[!t]
% \centering
% \includegraphics[width=1.98\columnwidth]{CheckGPT/img/boxplot2.png}\vspace{-3mm}
% \caption{Distribution of abstract lengths (\# of words): grey: HUM; red, green, blue, yellow: Prompt 1-4.}
% \label{fig:csdistlength}\vspace{-4mm}
% \end{figure*}

% The average lengths of GPT-generated abstracts are 187.3, 109.6, and 152.6 words for Tasks 1, 2, and 3, respectively. The average length of human-written abstracts is 183.6, 103.6, and 189.6. Note that we only consider the second half of the abstracts in Task 2.
% The average lengths of human-written abstracts and their second halves are 178.6 and 96.8. The average lengths of the GPT-generated abstracts in each task (GPT-WRI, -CPL, and -POL) are (182.5, 141.1, 162.2) for Prompt 1, (183.4, 144.3, 172.1) for Prompt 2, (172.6, 138.0, 169.2) for Prompt 3, and (204.3, 162.3, 190.6) for Prompt 4.
%The distributions of abstract lengths are shown in Figure~\ref{fig:distlength}, where we have some interesting observations: (1) In all three disciplines, the GPT-CPL abstracts are longer than the word limit, and thus the human-written abstracts. (2) The GPT-written abstracts are shorter than human-written abstracts using Prompt 1 and 3, but longer using Prompt 4. (3) The human-written abstracts in HSS are longer than the ones in CS and PHX.

%(1) human-written abstracts in physics are shorter than the other disciplines, while GPT-written abstracts in physics are longer than the other disciplines; (2) GPT-written abstracts are longer than human-written abstracts in physics but shorter in CS and HSS; (3) in all three disciplines, GPT-polished abstracts are shorter than human-written abstracts. %In general, ChatGPT's style is more concise than human authors, except in physics. 

%Please refer to Appendix~\ref{} for more details considering each subject.

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.9\columnwidth]{CheckGPT/tex/boxplot_sixcolumns.png}
% \caption{Distribution of abstract lengths.}
% \label{fig:distlength}
% \end{figure}



% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.95\columnwidth]{CheckGPT/tex/boxplot_physics.png}
% \caption{Distribution of abstract lengths in PHX.}
% \label{fig:phxdistlength}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.95\columnwidth]{CheckGPT/tex/boxplot_literal.png}
% \caption{Distribution of abstract lengths in HSS.}
% \label{fig:hssdistlength}
% \end{figure}

\begin{table}[t]
	\setlength{\tabcolsep}{0.38em}
 \caption{Performance of commercial GPT detectors on GPABench2. Red: detection accuracy <50\%, or average score on the wrong side of the decision threshold. T1/2/3: Task 1/2/3. GPT-WRI/CPL/POL: GPT-written/completed/polished abstracts.}\label{tab:otherdetectors} \vspace{-2mm}
 %\caption{Performance of open-source and commercial GPT detectors. }\label{tab:otherdetectors} 
    {
	\begin{tabular}{c|ccc|ccc|ccc}
        \hline
        
      \multirow{2}{*}{} & \multicolumn{3}{c|}{T1. GPT-WRI} &\multicolumn{3}{c|}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\
		\cline{2-10}
        & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline\hline
        \multicolumn{10}{c}{(a) Classification accuracy (in \%) of GPTZero.} \\\hline
GPT & \hic{30.3}	&	\hic{25.3}	&	72.0	&	\hic{17.0}	&	\hic{6.0}	&	\hic{43.7}	&	\hic{1.7}	&	\hic{2.3}	& \hic{20.3}	\\
Human	& 99.3	&	99.7 &	100   &	99.7	&	99.7	&	94.3	&	99.7	&	95.7	&	95.7	\\\hline\hline
    \multicolumn{10}{c}{(b1) Detection accuracy (in \%) of ZeroGPT} \\\hline
GPT & 67.4	&	68.4	&	92.3	&	\hic{25.3}	&	\hic{10}	&	62.4	&	\hic{3.3}	&	\hic{2.7}	&	\hic{24.7}	\\
Human	& 100	&	98.4	&	95	&	99.7	&	99.7	&	94.7	&	98.3	&	98.6	&	92.7 \\ \hline
    \multicolumn{10}{c}{(b2) Average score reported by ZeroGPT. 0:human, 8:GPT} \\\hline
GPT & 5.43	&	5.39	&	7.41	&	\hic{2.26}	&	\hic{0.97}	&	4.97	&	\hic{0.35}	&	\hic{0.29}	& \hic{2.15}	\\
Human	& 0.09	&  0.13 &	0.52   &	0.08	&	0.04	&	0.47	&	0.20	&	0.14	&	0.64	\\ \hline\hline
    \multicolumn{10}{c}{(c1) Detection accuracy (in \%) of OpenAI's detector} \\\hline
GPT & 80.7	 & 	70	 & 	63	 & 	63.7	 & 	\hic{23.7}	 & 	\hic{27.3}	 & 	\hic{6.3}	 & 	\hic{4.3}	 & 	\hic{6}  \\
Human	& 51.0	 & 	69.7	 & 	84.0	 & 	\hic{35.3}	 & 	59.7	 & 	79.6	 & 	50.7	 & 	69.0	 & 	88.0 \\
    \hline
    \multicolumn{10}{c}{(c2) Average score reported by OpenAI. 0:human, 4:GPT} \\\hline
GPT & 3.11	&	2.89	&	2.72	&	2.70	&	2.12	&	2.04	&	\hic{1.75}	&	\hic{1.59}	& \hic{1.52}	\\
Human	& 1.42	&  1.17 &	0.59   &	1.71	&	1.35	&	0.68	&	1.38	&	1.14	&	0.52	\\
    \hline   
        \end{tabular}
        }\vspace{-3mm}
\end{table}

\subsection{Benchmarking Online and Open-source ChatGPT Detectors}\label{sec:benchmark}\label{sec:comparison}

Several online commercial tools have been developed to detect AI-generated text. We are especially interested in them because they are the most accessible and easy-to-use detectors for ordinary users. We evaluate the accuracy of three representative online ChatGPT tools, GPTZero \cite{gptzero}, ZeroGPT \cite{zerogpt}, and OpenAI's classifier \cite{openaidetector}, over GPABench2. Due to a lack of API, slow responses, and high cost, we cannot run large-scale experiments. Instead, we randomly sampled 300 pairs of human-written and the corresponding GPT-generated abstracts for each task in each discipline, i.e., 2,400 pairs in total, and fed them to each detector. Their performance is summarized in Table \ref{tab:otherdetectors}. Note that, in Task 2 (GPT-completed abstracts), we only submitted the second half of each abstract to the detectors.  

From the performance summary in Table \ref{tab:otherdetectors} and the detailed results in Appendix \ref{apdx:benchmarking}, we have three observations: (1) all three detectors demonstrated modest to poor accuracy for GPT-GEN content; (2) the detectors have tendencies to classify GPT-generated text as human-written; and (3) the detection accuracy for GPT-GEN decreases significantly from Task 1 (GPT-WRI) to Task 3 (GPT-POL). Note that this experiment is not intended for comparison with CheckGPT. Since these models are not explicitly trained with academic data, their inaccuracy can be excused and directly comparing them with CheckGPT is unfair. Rather, we intend to use the results as a motivation for CheckGPT--generic detectors struggle in specific tasks, indicating limited transferability. The gap highlights the need for effective detectors for this niche domain with the potential to transfer to related domains. 

%\subsection{Benchmarking Open-source Detectors}\label{sec:benchmark}
A number of detectors have been proposed for LLM/ChatGPT-generated text. For a comparative study, we adopted 15 open-source detectors in the literature. 
Based on the design philosophy, we further categorize them into three groups: (a) \textit{Pre-trained detectors}. We directly adopt the trained models: HC3-Perplexity (HC3-PPL) \cite{guo2023close}, HC3-GLTR \cite{guo2023close}, HC3-Roberta (HC3-RBT) \cite{guo2023close}, OpenAI-Roberta (OpenAI-RBT) \cite{solaiman2019release, openairoberta}. (b) \textit{Statistics-based detectors}. They analyze the statistical differences between LLM and human-written text: Histogram-of-Likelihood Ranks (HLR) \cite{gehrmann2019gltr}, Rank \cite{mitchell2023detectgpt}, Log-Rank \cite{mitchell2023detectgpt}, Total Probability (TP) \cite{solaiman2019release} Perplexity (PPL) \cite{guo2023close}, Entropy \cite{gehrmann2019gltr, mitchell2023detectgpt}, DetectGPT \cite{mitchell2023detectgpt}.  (c) \textit{Fine-tuned Language Models}. They fine-tune the pre-trained language models for detection: BERT \cite{ippolito2020automatic}, DistillBERT \cite{he2023mgtbench}, and RoBERTa \cite{liu2023argugpt, guo2023close, wang2023m4, macko2023multitude}. We also include GPT-2, which is even larger with 355M parameters. Please refer to Appendix \ref{appdx:detectordetails} for more details. 

The statistics- and fine-tuning-based detectors are trained/tuned with the entire training set in GPABench2. We evaluate all the detectors on GPABench2 with samples generated by Prompt 1. From the results presented in Table~\ref{tab:opensourcedetector}, we observe the following: (1) The pre-trained detectors work poorly on GPABench2. The failure of the OpenAI detector can be attributed to the discrepancy in the target model, as it was designed for GPT-2. For HC3 detectors, their poor performance indicates the ineffectiveness of statistics-based methods (HC3-PPL, HC3-GLTR) and the limited transferability of RoBERTa (HC3-RBT). (2) The statistics-based detectors provide satisfactory performance in Task 1, however, they become mostly ineffective in Tasks 2 and 3. These results also indicate that GPT-polished content demonstrates significantly more statistical similarities to human-written text, especially at the lexicon level, e.g., word distributions, complexity, etc. (3) Fine-tuned language models with a native classification layer provide outstanding performance in most tasks, with slightly lower accuracy in Task 3. However, training or tuning the full BERT, RoBERTa, or GPT models is computationally expensive, e.g., it takes over 1,000 seconds to fine-tune BERT or RoBERTa for one epoch on an NVidia 4090 GPU, and more than 6,000 seconds for GPT-2. 

%, and the low transferability of fine-tuning LMs (RoBERTa), which highlights the advantage of our transferable \checkgpt. More details will be discussed in Section~\ref{subsec:newdomain}.

\begin{table}[t]
    \caption{Performance (F1-score) of open-source detectors on GPABench2. Values in blue: the best performance.}\label{tab:opensourcedetector}
    \setlength{\tabcolsep}{0.27em}
    \centering
    \vspace{-1mm}
    {\small 
	\begin{tabular}{c|ccc|ccc|ccc}
 \hline
        & \multicolumn{3}{c|}{T1. GPT-WRI} &\multicolumn{3}{c|}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\\hline
         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
           % \multicolumn{10}{c}{From top to bottom: Prompt 1, 2, 3, 4} \\\hline
           \multicolumn{10}{c}{(a) Pre-trained Detectors} \\\hline
        HC3-PPL & 0.760 & 0.794 & 0.854 & 0.688 & 0.686 & 0.763 & 0.665 & 0.668 & 0.682 \\
        HC3-GLTR  & 0.679 & 0.680 & 0.735 & 0.670 & 0.669 & 0.700 & 0.666 & 0.667 & 0.670 \\
        HC3-RBT & 0.710 & 0.788 & 0.795 & 0.726 & 0.753 & 0.786 & 0.722 & 0.746 & 0.805 \\
        OpenAI-RBT & 0.072 & 0.106 & 0.110 & 0.159 & 0.219 & 0.192 & 0.072 & 0.113 & 0.112 \\ \hline
        \multicolumn{10}{c}{(b) Statistics-based Detectors} \\\hline
        HLR & 0.910 & 0.917 & 0.902 & 0.792 & 0.757 & 0.841 & 0.608 & 0.602 & 0.682 \\
        Rank & 0.781 & 0.650 & 0.525 & 0.783 & 0.612 & 0.531 & 0.808 & 0.738 & 0.620\\
        Log-Rank & 0.911 & 0.919 & 0.895 & 0.794 & 0.764 & 0.843 & 0.626 & 0.608 & 0.679 \\
        TP & 0.913 & 0.924 & 0.894 & 0.797 & 0.778 & 0.847 & 0.632 & 0.622 & 0.686 \\
        PPL & 0.913 & 0.925 & 0.891 & 0.814 & 0.797 & 0.848 & 0.654 & 0.650 & 0.695\\
        Entropy & 0.803 & 0.851 & 0.745 & 0.697 & 0.708 & 0.738 & 0.558 & 0.593 & 0.633 \\
        DetectGPT & 0.790 & 0.722 & 0.768 & 0.685 & 0.693 & 0.766 & 0.616 & 0.588 & 0.630 \\ \hline
        % TDA &  \\  \hline
        \multicolumn{10}{c}{(c) Fine-tuned Language Models} \\\hline
        BERT & 0.999 & 0.999 & 0.998 & 0.992 & 0.983 & 0.992 & 0.983 & 0.984 & 0.966 \\
        DistillBERT & 0.999 & 0.999 & {\newc 0.999} & 0.990 & 0.992 & 0.975 & 0.977 & 0.989 & 0.973 \\
        RoBERTa & {\newc 0.999} & 0.999 & 0.997 & 0.970 & 0.995 & {\newc 0.995} & 0.981 & 0.993 & 0.967 \\ 
        GPT2 & 0.998 & 0.995 & 0.998 & 0.982 & 0.987 & 0.947 & 0.969 & 0.974 & 0.956 \\ 
        \hline
        CheckGPT & 0.999 & {\newc 1.000} & {\newc 0.999} & {\newc 0.996} & {\newc 0.995} & {\newc 0.995} & {\newc 0.993} & {\newc 0.994} & {\newc 0.993} \\ \hline        
        \end{tabular}
        } \vspace{-4mm}
\end{table}



%\subsection{Benchmarking Online Detection Tools}\label{sec:comparison}

%{\newc Many online commercial tools have been developed to detect AI-generated text. We are especially interested in them because they are the most accessible and easy-to-use approach for ordinary users, given ChatGPT's wide adoption and social impacts.} We evaluated the accuracy of three representative online ChatGPT tools, GPTZero \cite{gptzero}, ZeroGPT \cite{zerogpt}, and OpenAI's classifier \cite{openaidetector}, over our academic abstract dataset. Due to a lack of API, slow responses, and expenses, we cannot run large-scale experiments. Instead, we randomly sampled 300 pairs of human-written and the corresponding GPT-generated abstracts for each task in each discipline, i.e., 2,400 pairs in total, and fed them to each detector. Their performance is summarized in Table \ref{tab:otherdetectors}. Note that, in Task 2 (GPT-completed abstracts), we only submitted the second half of each abstract to the detectors.  



%From the performance summary in Table \ref{tab:otherdetectors} and the detailed results in Appendix \ref{apdx:benchmarking}, we have three observations: (1) all three detectors demonstrated modest to poor detection accuracy for GPT-GEN content; (2) the detectors have tendencies to classify GPT-generated text as human-written; and (3) the detection accuracy for GPT-GEN decreases significantly from Task 1 (GPT-WRI) to Task 3 (GPT-POL). Given that these models are not explicitly trained with academic datasets, their inadequacy can be excused. However, the results show that generic detectors struggle in specific tasks,
%to identify GPT-generated academic writing. 
%indicating a limited transferability. 
%The gap highlights the need for effective detectors for this niche domain with the potential to transfer to related domains.
%a detector specifically designed for this niche domain.



% \begin{table}[t]
% \centering
% 	\setlength{\tabcolsep}{0.2em}
%  \caption{Performance of open-source and commercial GPT detectors. Red: detection accuracy <50\%, or average score on the wrong side of the decision threshold. }\label{tab:otherdetectors} 
%  %\caption{Performance of open-source and commercial GPT detectors. }\label{tab:otherdetectors} 
%  \vspace{-2mm}
%     {\small
% 	\begin{tabular}{cccccccccc}
%         \hline
%       \multirow{2}{*}{} & \multicolumn{3}{c}{T1. GPT-WRI} &\multicolumn{3}{c}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\
% 		%\cline{2-10}
%         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
%         \multicolumn{10}{c}{(a) Classification accuracy (in \%) of GPTZero.} \\\hline
% GPT & \hic{30.3}	&	\hic{25.3}	&	72.0	&	\hic{17.0}	&	\hic{6.0}	&	\hic{43.7}	&	\hic{1.7}	&	\hic{2.3}	& \hic{20.3}	\\
% HUM	& 99.3	&	99.7 &	100   &	99.7	&	99.7	&	94.3	&	99.7	&	95.7	&	95.7	\\\hline
%     \multicolumn{10}{c}{(b1) Detection accuracy (in \%) of ZeroGPT} \\\hline
% GPT & 67.4	&	68.4	&	92.3	&	\hic{25.3}	&	\hic{10}	&	62.4	&	\hic{3.3}	&	\hic{2.7}	&	\hic{24.7}	\\
% HUM	& 100	&	98.4	&	95	&	99.7	&	99.7	&	94.7	&	98.3	&	98.6	&	92.7 \\ \hline
%     \multicolumn{10}{c}{(b2) Average score reported by ZeroGPT. 0:human, 8:GPT} \\\hline
% GPT & 5.43	&	5.39	&	7.41	&	\hic{2.26}	&	\hic{0.97}	&	4.97	&	\hic{0.35}	&	\hic{0.29}	& \hic{2.15}	\\
% HUM	& 0.09	&  0.13 &	0.52   &	0.08	&	0.04	&	0.47	&	0.20	&	0.14	&	0.64	\\ \hline
%     \multicolumn{10}{c}{(c.1) Detection accuracy (in \%) of OpenAI's detector} \\\hline
% GPT & 80.7	 & 	70	 & 	63	 & 	63.7	 & 	\hic{23.7}	 & 	\hic{27.3}	 & 	\hic{6.3}	 & 	\hic{4.3}	 & 	\hic{6}  \\
% HUM	& 51.0	 & 	69.7	 & 	84.0	 & 	\hic{35.3}	 & 	59.7	 & 	79.6	 & 	50.7	 & 	69.0	 & 	88.0 \\
%     \hline
%     \multicolumn{10}{c}{(c.2) Average score reported by OpenAI. 0:human, 4:GPT} \\\hline
% GPT & 3.11	&	2.89	&	2.72	&	2.70	&	2.12	&	2.04	&	\hic{1.75}	&	\hic{1.59}	& \hic{1.52}	\\
% HUM	& 1.42	&  1.17 &	0.59   &	1.71	&	1.35	&	0.68	&	1.38	&	1.14	&	0.52	\\
%     \hline    
%         \end{tabular}}
%          \vspace{-4mm}
% \end{table}

% \begin{table}[t]
% 	\setlength{\tabcolsep}{0.25em}
%  \caption{Open-source and commercial GPT detectors. }\label{tab:otherdetectors} 
 
%  \textbf{(a) Classification accuracy (in \%) of GPTZero.}\vspace{1mm}
    
% 	\begin{tabular}{cccccccccc}
%       \multirow{2}{*}{} & \multicolumn{3}{c}{Task 1. GEN} &\multicolumn{3}{c}{Task 2. CPL}  &\multicolumn{3}{c}{Task 3. POL}\\
% 		\cline{2-10}
%         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
% GPT & 30.3	&	25.3	&	72.0	&	17.0	&	6.0	&	43.7	&	1.7	&	2.3	& 20.3	\\
% Human	& 99.3	&	99.7 &	100   &	99.7	&	99.7	&	94.3	&	99.7	&	95.7	&	95.7	\\
%         \end{tabular}
        
% \vspace{2mm}
% \textbf{(b) Average score reported by ZeroGPT: 8=GPT; 0=human.}\vspace{1mm}

%         	\begin{tabular}{cccccccccc}
%       \multirow{2}{*}{} & \multicolumn{3}{c}{Task 1. GEN} &\multicolumn{3}{c}{Task 2. CPL}  &\multicolumn{3}{c}{Task 3. POL}\\
% 		\cline{2-10}
%         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
% GPT & 5.43	&	5.39	&	7.41	&	2.26	&	0.97	&	4.97	&	0.35	&	0.28	& 2.15	\\
% Human	& 0.09	&  0.13 &	0.52   &	0.08	&	0.04	&	0.47	&	0.20	&	0.14	&	0.64	\\
%         \end{tabular}
% \end{table}








==> CheckGPT/tex/evaluation.tex <==
\section{Experiments}\label{sec:exp}
% Linguistic Analysis - SVM
% TP and FP 2/3-gram
%\subsection{Settings and Metrics}

\subsection{Settings and Metrics}

We implement \checkgpt~with PyTorch 1.13.1 in Python 3.9.1 on Ubuntu 22.04. The pre-trained RoBERTa is adopted from \cite{robertahuggingface}. All the experiments were conducted on an Nvidia 2080Ti GPU and an Intel i9-9900k CPU. We use GPABench2 for most of the experiments. \checkgpt~is trained with an initial learning rate of 2e-4, a batch size of 256, and an early-stop strategy to finish training when the validation loss stays flat for a predefined number of epochs. %{\newc Otherwise specified, we will use Prompt 1, on which \checkgpt~has the most challenges.}

When we consider \checkgpt~as GPT-generated content detector, the \textit{true positive} rate ($TPR=\frac{TP}{TP+FN}$) is the proportion of correctly detected GPT-generated abstracts out of all GPT-generated abstracts, i.e., the accuracy in classifying GPT-generated text. The \textit{true negative} rate ($TNR=\frac{TN}{TN+FP}$), is the proportion of correctly identified human-written abstracts out of all human-written abstracts, i.e. the accuracy in classifying human-written text. The overall accuracy is defined as the proportion of correctly classified samples over all the testing samples: $Acc=\frac{TP+TN}{TP+FP+TN+FN}$. 
% We implement \checkgpt~with PyTorch 1.13.1 in Python 3.9.1 on Ubuntu 22.04, running on an Nvidia 2080Ti GPU and an Intel i9-9900k CPU. The pre-trained RoBERTa is adopted from \citealp{robertahuggingface}. See Appendix~\ref{apdx:settings} for more details.

%TPR denotes the proportion of correctly identified GPT-GEN abstracts out of all GPT-GEN abstracts. TNR is the proportion of correctly identified HUM abstracts out of all HUM abstracts.

%For all the evaluations, we categorize GPT-generated abstracts as positive cases and use the True Positive Rate (TPR) to assess correctness. Similarly, True Negative Rate (TNR) applies to human-written abstracts. TNR is the proportion of correctly identified HUM abstracts out of all HUM abstracts.

% When we consider \checkgpt~as GPT-generated content detector, the \textit{true positive} rate ($TPR=\frac{TP}{TP+FN}$) is the proportion of correctly detected GPT-generated abstracts out of all GPT-generated abstracts, i.e., the accuracy in classifying GPT-generated text. The \textit{true negative} rate ($TNR=\frac{TN}{TN+FP}$), is the proportion of correctly identified human-written abstracts out of all human-written abstracts, i.e., the accuracy in classifying human-written text. The overall classification accuracy of \checkgpt~is defined as the proportion of correctly classified samples over all the testing samples: $Acc=\frac{TP+TN}{TP+FP+TN+FN}$. 

\subsection{Task- and Discipline-specific Classifiers}\label{sec:baselineperf}

\begin{table}[t]
	\caption{\checkgpt's performance (in \%) for each task, discipline, and prompt: TPR, TNR, accuracy (Acc).}\label{tab:checkgpt}
    \setlength{\tabcolsep}{0.3em}
    \centering
    \vspace{-2mm}
    {\small
	\begin{tabular}{c|ccc|ccc|ccc}
        \hline
       & \multicolumn{3}{c|}{T1. GPT-WRI} &\multicolumn{3}{c|}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\\cline{2-10}
         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
           % \multicolumn{10}{c}{From top to bottom: Prompt 1, 2, 3, 4} \\\hline
           \multicolumn{10}{c}{Prompt 1} \\\hline
TPR & 99.95 & 100.0 & 99.94 & 99.58 & 99.50 & 99.48 & 99.23 & 99.31 & 99.22 \\
TNR & 99.97 & 100.0 & 100.0 & 99.70 & 99.57 & 99.67 & 99.33 & 99.40 & 99.39 \\
ACC & 99.96 & 100.0 & 99.97 & 99.64 & 99.54 & 99.58 & 99.28 & 99.36 & 99.31 \\
\hline


\multicolumn{10}{c}{Prompt 2} \\\hline
TPR & 99.99 & 100.0 & 100.0 & 99.63 & 99.50 & 99.65 & 99.23 & 99.50 & 99.32 \\
TNR & 99.99 & 100.0 & 99.98 & 99.75 & 99.63 & 99.68 & 99.33 & 99.51 & 99.40 \\
ACC & 99.99 & 100.0 & 99.99 & 99.69 & 99.57 & 99.67 & 99.28 & 99.51 & 99.36 \\
\hline


\multicolumn{10}{c}{Prompt 3} \\\hline
TPR & 99.97 & 99.99 & 99.96 & 99.78 & 99.68 & 99.67 & 99.33 & 99.35 & 99.46 \\
TNR & 100.0 & 100.0 & 99.98 & 99.76 & 99.79 & 99.71 & 99.34 & 99.68 & 99.36 \\
ACC & 99.98 & 100.0 & 99.97 & 99.77 & 99.74 & 99.69 & 99.34 & 99.52 & 99.41 \\
\hline


\multicolumn{10}{c}{Prompt 4} \\\hline
TPR & 100.0 & 99.99 & 99.96 & 99.76 & 99.71 & 99.67 & 99.41 & 99.61 & 99.47 \\
TNR & 99.99 & 100.0 & 99.99 & 99.77 & 99.78 & 99.88 & 99.60 & 99.69 & 99.50 \\
ACC & 100.0 & 100.0 & 99.98 & 99.77 & 99.75 & 99.78 & 99.51 & 99.65 & 99.49 \\
\hline

        \end{tabular}} \vspace{-4mm}

% 1literal， Epoch:0, Test accuracy: 99.9300%, Acc_GPT: 99.9402%, Acc_Human: 99.9197%
% 2literal， Epoch:0, Test accuracy: 98.7850%, Acc_GPT: 98.5750%, Acc_Human: 98.9965%
% 3literal， Epoch:0, Test accuracy: 98.4700%, Acc_GPT: 98.4454%, Acc_Human: 98.4947%

% new table

%         	\begin{tabular}{cccccccccc}
%       \multirow{2}{*}{} & \multicolumn{3}{c}{T1. GPT-WRI} &\multicolumn{3}{c}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\
% 		\cline{2-10}
%         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
% GPT     & 	&		&	&		&		&		&		&		& 	\\
% Human	& 	&		&	&		&		&		&		&		& 	\\ \hline
% Avg. & 99.97 &	99.99	&	99.93	&	99.32	&	97.93	&	98.79	&	98.39	&	99.08	&	98.47	\\
% \end{tabular}
\end{table}

We first evaluate \checkgpt~at the finest granularity: one classifier for each discipline, task, and prompt combination. We use an 80\%-20\% train-test split on the main GPABench2 dataset: 80K samples (40K each of GPT and HUM) for training and 20K for testing. 
Training takes an average of 120s per epoch, while testing takes about 0.03s per sample. We report the classification accuracy in Table~\ref{tab:checkgpt}. 

%TPR denotes the proportion of correctly identified GPT-GEN abstracts out of all GPT-GEN abstracts. TNR is the proportion of correctly identified HUM abstracts out of all HUM abstracts.


\checkgpt~achieves very high accuracy in all cases. The detection accuracy for Task 1 (abstracts entirely written by ChatGPT) is higher than 99.9\% across all disciplines/prompts.  
Task 2, where only the second halves of the abstracts are checked, has slightly lower accuracy, which is explained by shorter text lengths and better writing by ChatGPT given more seed data.
The accuracy of Task 3, which is most challenging for the open-source and commercial detectors (Sec. \ref{sec:benchmark}), is between 99.28\% and 99.65\%. 
%In conclusion, the task-specific discipline-specific classifiers demonstrate outstanding performance in distinguishing human-written and GPT-generated abstracts, even for tasks that pose difficulties for the other SOTA detectors. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.98\columnwidth]{CheckGPT/img/train_loss.png}\vspace{-3mm}
\caption{Training losses of the task-specific and discipline-specific classifiers.}\vspace{-2mm}
\label{fig:trainloss} \vspace{-2mm}
\end{figure}

Figure \ref{fig:trainloss} shows the training losses (Prompt 1). Task 1 models rapidly grasp simple features like lexical characteristics, while Tasks 2 and 3 are more difficult. In most cases, HSS is more challenging, which implies that ChatGPT does a better job mimicking human-written style in these topics. Task 2 is the outlier, where the samples in PHX are significantly shorter and thus harder to distinguish.
% A different pattern is observed in Task 2, as the short samples in physics introduce additional challenges to the classifier.  

% Finally, we use t-Distributed Stochastic Neighbor Embedding (t-SNE) %\cite{van2008visualizing} 
% to analyze the vector representations extracted from the last layer and discuss the observations in Appendix \ref{apdx:tsne}. 

We randomly select 2,000 CS abstracts from each task/label, and then use t-Distributed Stochastic Neighbor Embedding (t-SNE) \cite{van2008visualizing} to map the 1024-D feature vectors from the last dense layer of the BiLSTM module into a 3-D space, as shown in Figure~\ref{fig:visualize}. The figure shows that: (a) GPT-written abstracts form a dense cluster (consistent vocabulary, writing style, and semantic features), which is different from the varied distribution of human-written samples. (b) GPT-completed abstracts (Task 2) are significantly more diverse than the GPT-written ones. While their representations are closer to the human-written samples, a distinct gap remains. (c) GPT-polished samples are scattered and intertwined with human-written samples, demonstrating the challenges in Task 3.

\begin{figure}[!t]
\centering
\includegraphics[width=0.98\columnwidth]{CheckGPT/img/visualize1.png}\vspace{-3mm}
\caption{Feature space distribution of human-written (green) and GPT-generated (red) abstracts.}
\label{fig:visualize}
\end{figure}

%The takeaways are: (a) GPT-written abstracts form a dense cluster, which is different from the varied distribution of the human-written samples, suggesting a consistent vocabulary, writing style, and semantic features. (b) GPT-completed abstracts are significantly more diverse than the GPT-written ones. While their representations are closer to the human-written samples, a distinct gap still remains. (c)) GPT-polished samples are scattered and intertwined with the human-written samples, demonstrating the difficulty in separating these two categories. 

%Finally, we visualize the distribution of the human-written and GPT-generated abstracts in the feature space. We randomly select 2,000 CS abstracts from each task and each label, extract their vector representations right from the last linear layer of the classification head, and employ the t-Distributed Stochastic Neighbor Embedding (t-SNE) \cite{van2008visualizing} to visualize the data points in a 3-dimensional space, as shown in Figure \ref{fig:visualize}.%, where human-written samples are in green and the GPT-generated samples are in red. 
% As we can see, the GPT-written abstracts in Figure \ref{fig:visualize} (a) are highly clustered, which implies that the vocabulary, the writing style, and the semantic features of these abstracts are very consistent so that they are easily distinguishable from the human-written abstracts, which appear to be more diverse in the feature space. The GPT-completed samples in Figure \ref{fig:visualize} (b) are shown to be significantly more diverse than the GPT-written samples. While they are also closer to the human-written samples in the feature space, there is still a clear separation between the two classes of samples. Finally, the GPT-polished samples in Figure \ref{fig:visualize} (c) appear scattered, where some data points appear to be blended with the human-written samples in a 3-dimensional space, demonstrating the difficulty in separating these two classes. 

\noindent\textbf{\em Ablation study.}  We compare the current design of \checkgpt~with several alternatives. %As a scrappy baseline, GLoVe with a two-layer MLP (size 1024) yields an unsatisfying F1-score of 0.755 on Task 3. 
We first keep the classification head in \checkgpt~and replace the representation module with GLoVe6B-100d \cite{pennington2014glove} or pre-trained BERT. As shown in Table \ref{tab:ablation}, there is a slight performance drop. We then keep the representation module and replace the classifier with: the default classification head for RoBERTa (RCH) \citet{robertahuggingface}, and its variant with global average pooling (MLP-Pool; \citealp{lin2013network, keraspool}); an AlexNet-like CNN \cite{krizhevsky2012imagenet} with five convolutional layers, and (4) a basic BiLSTM without attention.  As shown in Table \ref{tab:ablation}, \checkgpt~achieves the best accuracy. 

%The results, including the parameter amounts, average inference time (out of 1,000 tests), and accuracy, are shown in Table \ref{tab:ablation}. 

%Experiments are repeated under the same settings on the challenging CS-Prompt-1.

\begin{table}[t]
\caption{Comparison with other design choices.} \label{tab:ablation}
\setlength{\tabcolsep}{0.3em}
\centering
\vspace{-3mm}
{\small
\begin{tabular}{c|c|ccc}
\hline
\multirow{2}{*}{Model} & Para & \multicolumn{3}{c}{Acc(\%)} \\ \cline{3-5}
 & Size & Task 1 & Task 2 & Task 3 \\\hline
 GLoVe + \checkgpt~classifier & - & 99.77 & 98.34 & 95.90 \\
 BERT + \checkgpt~classifier & - & 99.90 & 99.28 & 97.81 \\\hline
\checkgpt~representation + RCH & 1.05M & 99.80 & 97.70 & 94.08 \\
\checkgpt~representation + MLP-Pool & 1.05M & 99.87 & 98.62 & 95.93 \\
\checkgpt~representation + CNN & 3.33M & 99.80 & 98.47 & 96.49 \\
\checkgpt~rep. + BiLSTM w/o attention & 4.21M & 99.91 & 99.54 & 98.92 \\\hline
% BiLSTM w attention & 4.21M & 99.96 & 99.60 & 99.17 \\\hline%\hline
% BiGRU w attention & 4.21M & 99.94 & 99.64 & 99.28\\\hline
\checkgpt & 4.21M & 99.98 & 99.72 & 99.39 \\
% {\newc \checkgpt~(GRU)} & 4.21M & 99.94 & 99.64 & 99.28 \\
\hline
\end{tabular}} \vspace{-3mm}
\end{table}

% \begin{table}[t]
% \caption{Comparison with other design choices.} \label{tab:ablation}
% \setlength{\tabcolsep}{0.3em}
% \centering
% \vspace{-3mm}
% {\small
% \begin{tabular}{c|c|ccc}
% \multirow{2}{*}{Model} & Para & \multicolumn{3}{c}{Acc(\%)} \\ \cline{3-5}
%  & Size & Task 1 & Task 2 & Task 3 \\\hline
% \multicolumn{5}{c}{(a) Other representation module + \checkgpt~classifier}\\\hline
%  GLoVe & - & 99.77 & 98.34 & 95.90 \\
%  BERT & - & 99.90 & 99.28 & 97.81 \\\hline
% \multicolumn{5}{c}{(b) \checkgpt~representation module + other classifier}\\\hline
% RCH & 1.05M & 99.80 & 97.70 & 94.08 \\
% MLP-Pool & 1.05M & 99.87 & 98.62 & 95.93 \\
% CNN & 3.33M & 99.80 & 98.47 & 96.49 \\
% BiLSTM w/o attention & 4.21M & 99.91 & 99.54 & 98.92 \\\hline
% % BiLSTM w attention & 4.21M & 99.96 & 99.60 & 99.17 \\\hline%\hline
% % BiGRU w attention & 4.21M & 99.94 & 99.64 & 99.28\\\hline
% BiLSTM w/ attention & 4.21M & 99.96 & 99.64 & 99.28 \\
% % {\newc \checkgpt~(GRU)} & 4.21M & 99.94 & 99.64 & 99.28 \\

% \end{tabular}} \vspace{-3mm}
% \end{table}
% ('2.16 GMac', '4.21 M')
% ('1.05 MMac', '1.05 M')
% ('1.05 MMac', '1.05 M')
% ('1.23 GMac', '3.33 M')
% ('2.16 GMac', '4.21 M')




\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{CheckGPT/img/heatmap_2col.jpg}\vspace{-2mm}
\caption{\checkgpt's transferability across disciplines and tasks: (a) without fine-tuning, (b): tuned with 5\% data from the train set. 1C: Task 1 GPT-WRI+CS; 2P: Task 2 GPT-CPL+PHX; 3H: GPT-POL+HSS. }
\label{fig:transfer} \vspace{-2mm}
\end{figure}

\subsection{Transferability across Tasks, Disciplines, and Prompts}\label{sec:transfer}
We evaluate \checkgpt's capability of cross-prompt, cross-task, and cross-disciplinary generalization. First, we train nine cross-prompt models (one model for each task and discipline as shown in Table \ref{tab:unified} (a)) to evaluate testing samples from \textbf{other} tasks and disciplines, \textit{without model fine-tuning}. In Figure \ref{fig:transfer} (a), each value demonstrates the F1-score using the model from the task/discipline denoted on the x-axis to test samples from the task/discipline on the y-axis. From the figure, we observe the following:

%\begin{itemize}[noitemsep, topsep=1mm, left=0pt]
\noindent$\bullet~$ \checkgpt~is adaptable \textit{across disciplines}. \checkgpt~achieves $\geq$0.978 F1-score on \textit{cross-discipline} data from the \textit{same task}.

\noindent$\bullet~$ \checkgpt~is less adaptable \textit{across tasks}. In particular, the models trained in Task 1 demonstrate low performance with testing samples from the other tasks, while the models from Task 2 are also less capable of handling Task 3 (GPT-POL) data.

\noindent$\bullet~$ The models trained in Task 3 demonstrate solid performance with testing samples from Tasks 1 and 2. It implies that Task 3 could be the most difficult, and the models have learned subtle but inherent features of AIGC.

% \checkgpt~achieves $\geq$0.978 F1-score on \textit{cross-discipline} data from the \textit{same task}. However, \checkgpt~is less adaptable \textit{across tasks}. In particular, Task 1 models perform the worst on data from Task 3. Task 3 models demonstrate solid performance on other Tasks. It implies that \checkgpt~learns subtle but inherent features of AIGC in the most challenging Task 3.

We then fine-tune the last linear layer of each model with the data in the target domain. As shown in Figure \ref{fig:transfer} (b), tuning with as few as 5\% of data (2K samples) increases the classification F1-score to 0.97+ in all cases, while the distribution patterns of the F-1 scores remain similar to Figure \ref{fig:transfer}(a). 

%we use our existing data to evaluate how \checkgpt~could be used to handle research paper abstracts from other disciplines with and without transfer learning. 



\begin{table}[t]
	\caption{TPR and TNR (in \%) of the unified classifiers.}\label{tab:unified}
    \setlength{\tabcolsep}{0.39em}
    \centering
    \vspace{-3mm}
    {\small
	\begin{tabular}{c|ccc|ccc|ccc}
    \hline
        & \multicolumn{3}{c|}{T1. GPT-WRI} &\multicolumn{3}{c|}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\ \cline{2-10}
         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\ \hline
         \multicolumn{10}{c}{(a) Cross-prompt Classifiers}\\\hline
% TPR & 99.95 & 99.98 & 99.95 & 99.50 & 99.42 & 99.42 & 98.99 & 99.21 & 99.01 \\
% TNR & 100.0 & 99.99 & 99.98 & 99.63 & 99.65 & 99.61 & 98.95 & 99.22 & 99.22 \\
TPR & 99.99 & 99.99 & 99.99 & 99.84 & 99.87 & 99.78 & 99.74 & 99.75 & 99.74 \\
TNR & 99.97 & 100.0 & 99.97 & 99.52 & 99.43 & 99.51 & 98.87 & 99.31 & 98.90 \\
\hline


 \multicolumn{10}{c}{(b) Cross-prompt Cross-disciplinary Classifiers}\\\hline
% TPR & 99.94 & 99.95 & 99.88 & 99.41 & 99.25 & 99.31 & 98.74 & 99.14 & 98.70 \\
% TNR & 99.97 & 100.0 & 99.97 & 99.54 & 99.59 & 99.30 & 98.74 & 99.25 & 98.92 \\
TPR & 99.99 & 99.99 & 99.99 & 99.82 & 99.72 & 99.72 & 99.62 & 99.73 & 99.62 \\
TNR & 99.99 & 100.0 & 99.99 & 99.66 & 99.67 & 99.72 & 99.10 & 99.58 & 99.24 \\
\hline

         \multicolumn{10}{c}{(c) Cross-prompt \& -task \& -disciplinary Classifier}\\\hline
% TPR & 99.98 & 99.97 & 99.99 & 98.96 & 98.67 & 98.95 & 96.95 & 97.53 & 97.15 \\
% TNR & 98.24 & 99.17 & 98.46 & 98.95 & 99.37 & 98.98 & 98.24 & 99.17 & 98.46 \\
TPR & 100.0 & 100.0 & 100.0 & 99.81 & 99.77 & 99.80 & 99.58 & 99.76 & 99.65 \\
TNR & 99.16 & 99.46 & 99.27 & 99.47 & 99.45 & 99.55 & 99.16 & 99.46 & 99.27 \\
\hline
        \end{tabular}} %\vspace{-5mm}
\end{table}
% 1cs， Epoch:0, Test accuracy: 99.9800%, Acc_GPT: 99.9799%, Acc_Human: 99.9801%
% 2cs， Epoch:0, Test accuracy: 99.2850%, Acc_GPT: 99.3477%, Acc_Human: 99.2227%
% 3cs， Epoch:0, Test accuracy: 98.6800%, Acc_GPT: 98.9262%, Acc_Human: 98.4355%
% 1physics， Epoch:0, Test accuracy: 99.9950%, Acc_GPT: 100.0000%, Acc_Human: 99.9900%
% 2physics， Epoch:0, Test accuracy: 97.8850%, Acc_GPT: 97.4736%, Acc_Human: 98.2911%
% 3physics， Epoch:0, Test accuracy: 99.4150%, Acc_GPT: 99.3979%, Acc_Human: 99.4320%
% 1literal， Epoch:0, Test accuracy: 99.9350%, Acc_GPT: 99.9402%, Acc_Human: 99.9298%
% 2literal， Epoch:0, Test accuracy: 98.8100%, Acc_GPT: 98.3956%, Acc_Human: 99.2273%
% 3literal， Epoch:0, Test accuracy: 98.7900%, Acc_GPT: 98.7544%, Acc_Human: 98.8259%

% 1cs， Epoch:0, Test accuracy: 99.6150%, Acc_GPT: 100.0000%, Acc_Human: 99.2327%
% 2cs， Epoch:0, Test accuracy: 99.0800%, Acc_GPT: 99.3578%, Acc_Human: 98.8042%
% 3cs， Epoch:0, Test accuracy: 98.7200%, Acc_GPT: 98.2037%, Acc_Human: 99.2327%
% 1physics， Epoch:0, Test accuracy: 99.8650%, Acc_GPT: 100.0000%, Acc_Human: 99.7309%
% 2physics， Epoch:0, Test accuracy: 98.0500%, Acc_GPT: 97.4635%, Acc_Human: 98.6289%
% 3physics， Epoch:0, Test accuracy: 99.4600%, Acc_GPT: 99.0768%, Acc_Human: 99.8406%
% 1literal， Epoch:0, Test accuracy: 99.8200%, Acc_GPT: 99.9701%, Acc_Human: 99.6688%
% 2literal， Epoch:0, Test accuracy: 98.8400%, Acc_GPT: 98.8839%, Acc_Human: 98.7958%
% 3literal， Epoch:0, Test accuracy: 99.1150%, Acc_GPT: 98.5551%, Acc_Human: 99.6789%


\noindent\textbf{\em Prompt Transferability.} To assess \checkgpt's generalizability over domain shifts caused by ChatGPT prompts, we train it with data from 3 prompts and test it with samples from the fourth prompt. As shown in Table~\ref{tab:3to1},  \checkgpt~is highly transferable across prompts. Notably, testing accuracy for Prompt 1 is usually the lowest, which is explained by the fact that Prompt provided minimal context to ChatGPT so that the outputs are most diverse. 

%which is the most challenging by providing minimal context and information.

\begin{table}[t]
	\caption{TPR and TNR (in \%) of cross-prompt testing.}\label{tab:3to1}
    \setlength{\tabcolsep}{0.3em}
    \centering
    \vspace{-3mm}
    {\small
	\begin{tabular}{c|ccc|ccc|ccc}
    \hline
        & \multicolumn{3}{c|}{T1. GPT-WRI} &\multicolumn{3}{c|}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\ \cline{2-10}
         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
         \multicolumn{10}{c}{(a) Train with Prompts 2, 3, 4; test with Prompt 1}\\\hline
TPR & 99.73 & 99.91 & 99.63 & 99.43 & 99.31 & 99.54 & 97.73 & 98.47 & 98.00 \\
TNR & 99.89 & 99.99 & 99.95 & 99.35 & 99.42 & 99.19 & 98.54 & 99.00 & 98.99 \\
\hline


\multicolumn{10}{c}{(b) Train with Prompts 1, 3, 4; test with Prompt 2}\\\hline
TPR & 99.46 & 99.83 & 99.59 & 99.63 & 99.50 & 99.55 & 98.82 & 99.18 & 99.59 \\
TNR & 99.89 & 99.81 & 99.85 & 99.14 & 99.40 & 99.20 & 99.23 & 99.39 & 98.87 \\
\hline


\multicolumn{10}{c}{(c) Train with Prompts 1, 2, 4; test with Prompt 3}\\\hline
TPR & 99.99 & 99.99 & 99.97 & 99.31 & 99.51 & 99.60 & 99.34 & 99.75 & 99.68 \\
TNR & 99.87 & 99.92 & 99.89 & 99.49 & 99.46 & 99.29 & 98.86 & 98.98 & 98.80 \\
\hline

\multicolumn{10}{c}{(d) Train with Prompts 1, 2, 3; test with Prompt 4}\\\hline
TPR & 99.98 & 99.95 & 99.95 & 99.67 & 99.39 & 99.51 & 99.75 & 99.63 & 99.79 \\
TNR & 99.79 & 99.91 & 99.82 & 99.06 & 99.41 & 99.35 & 98.47 & 98.99 & 98.79 \\
\hline
\end{tabular}}\vspace{-2mm}
\end{table}


%Task 1&2&3: Test accuracy: 99.1256%, Acc_GPT: 98.9506%, Acc_Human: 99.2999%

\noindent\textbf{\em The Unified Classifiers.} We evaluate \checkgpt~by sampling data from all prompts (train with 80K GPT samples for each task/discipline) and show the classification accuracy in Table~\ref{tab:unified}~(a). We then combine data across disciplines (Table~\ref{tab:unified} (b)) and further across all tasks 
(Table~\ref{tab:unified} (c)). In summary, unified training slightly improves TPR, especially for difficult tasks, e.g., GPT-POL in CS.
% We train a cross-discipline classifier for each task with the training samples from all the disciplines, and test it against the remaining discipline. and report the true positive and true negative rates in Table~\ref{tab:unified} (a). Finally, we train a unified cross-task cross-discipline classifier for all the tasks and disciplines.  The true positive and true negative rates are reported in Table~\ref{tab:unified} (b). In summary, both unified classifiers (a) and (b) perform well in the testing of each task-discipline experiment. Specifically, the unified training helps boost individual task performance, such as the difficult GPT-POL in HSS. These experiments further suggest the feasibility of developing general detecting algorithms in academia.


\noindent\textbf{\em The Multi-Task Classifier.} Finally, we investigate whether \checkgpt~is able to further distinguish the difference among the three tasks. To do this, we turn \checkgpt~into a unified, 4-ary classifier to distinguish HUM, GPT-WRI, GPT-CPL, and GPT-POL abstracts. \checkgpt~achieved a 98.51\% accuracy, with 98.75\%, 99.39\%, 97.69\%, and 98.24\% for HUM, GPT-WRI, GPT-CPL, and GPT-POL, respectively. \checkgpt's accuracy drops slightly due to the challenges of multi-label classification, but it can still catch the subtle differences in three tasks well. 






%\noindent\textbf{Task-specific Cross-discipline Classifiers.} We train a cross-discipline classifier for each task with the training samples from all three disciplines in the same task. We test each classifier with the testing samples in each discipline and report the true positive and true negative rates in Table~\ref{tab:unified} (a). 

%\noindent\textbf{The Unified Classifier.} Finally, we train a cross-task, cross-discipline classifier for all the tasks and disciplines.  The true positive and true negative rates are reported in Table~\ref{tab:unified} (b). 




\subsection{Transferability to New Domains}\label{subsec:newdomain}
%\noindent\textbf{\checkgpt~for other Domains.}

\textbf{\em Other academic writing purposes.} While our GPABench2 focuses on abstracts of research papers, ChatGPT can be used for other writing purposes, e.g., other sections of papers. While paper abstracts are almost always publicly available, the full papers are often restricted by copyright. Web scraping is not allowed even for open-access papers. Thus, we do not attempt to include human-written full papers in GPABench2. Instead, we provide ChatGPT with titles and ask it to write introduction, background, and conclusion sections for the title (similar to Task 1).
For each discipline and section, we collect 10,000 samples using the titles from GPABench2 (90,000 in total). We apply the cross-prompt cross-discipline \checkgpt~(Sec. \ref{sec:transfer}) on the new sections. As shown in Table \ref{tab:otherpurpose}, \checkgpt~maintains 99.9\% accuracy for all the sections. This shows the high potential of \checkgpt~for general academic writing. 


%\textbf{\em Different academic writing purposes.} While our GPABench2 focuses on the paper abstracts, ChatGPT can be used for other writing purposes, i.e., paper sections. Notably, unlike paper abstracts, which are almost always open-source and publicly available, publishers usually limit access to the paper content. Even granted access, e.g., to open-source papers, scraping inside the paper files is not a responsible practice. Thus, due to copyright and ethical considerations, we have not built datasets over paper sections other than abstracts. However, it is still feasible to evaluate CheckGPT on various writing purposes. Specifically, we ask ChatGPT to generate writing for three other purposes: (1) Introduction. (2) Background. (3) Conclusion. We provide ChatGPT with the paper titles similarly to collecting data for Task 1 (GPT-WRI). For each discipline and purpose, we collect 10,000 samples based on the test set in GPABench2, which totals 90,000. We apply the cross-prompt cross-discipline \checkgpt~classifiers (Sec. \ref{sec:transfer}) on the new purposes. As shown in Table \ref{tab:otherpurpose}, the performance of \checkgpt~has not been negatively affected by the transfer of writing purposes. This shows the high potential of \checkgpt~for general but academic writing purposes. 

\begin{table}[t]
	\caption{TPR (in \%) of other writing purposes.}\label{tab:otherpurpose}
    \setlength{\tabcolsep}{0.3em}
    \centering
    \vspace{-3mm}
    {
	\begin{tabular}{c|ccc|ccc|ccc}
 \hline
        & \multicolumn{3}{c|}{Introduction} &\multicolumn{3}{c|}{Background}  &\multicolumn{3}{c}{Conclusion}\\ \cline{2-10}
         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\ \hline
TPR & 99.99 & 100.0 & 100.0 & 99.99 & 100.0 & 99.98 & 100.0 & 100.0 & 100.0 \\
\hline
        \end{tabular}}
\end{table}


\noindent
\textbf{\em Classic NLP Datasets.} We evaluate \checkgpt~with three NLP datasets: Wiki Abstracts (1,500 random samples from \citealp{brummer2016dbpedia}), ASAP Essays \cite{hewlettessaydataset}, and BBC News \cite{greene06icml}. In ASAP Essays, we selected two different tasks: ``letters stating opinions on computers'' (Essay-C), and ``stories about patience'' (Essay-P). We adopted the original instructions in \citet{hewlettessaydataset} for Task 1 and designed the prompts for the other tasks and datasets (see Appendix~\ref{apdx:newdomain} for details).
%Tasks are defined in the same way as previous experiments. GPT-written articles in Task 1 are generated with an article title in the prompt. GPT-completed and GPT-polished articles are generated using human-written articles as seeds. 
We apply the cross-prompt cross-discipline \checkgpt~classifiers (Sec. \ref{sec:transfer}) on the new domains. As shown in Table \ref{tab:otherdataset}, \checkgpt~shows solid performance, especially on objective, structural, or argumentative writing like news and opinions. When the last layer of \checkgpt~is tuned with 100 samples (50 for each label) from each domain, it achieves significantly higher accuracy. %Note that we use the same data for testing before and after fine-tuning.

\noindent
\textbf{\em SOTA ChatGPT Datasets in the Literature.}
%As we have demonstrated the transferability of \checkgpt~within GPABench2, 
We further evaluate \checkgpt~on five ChatGPT datasets in the literature that cover 15 domains. %This rules out the possibility that the observed transferability is rooted in biases in GPABench2.
We adopted the following datasets: student essays in ArguGPT \cite{liu2023argugpt}; Finance, Medicine, OpenQA, Reddit, and Wikipedia in HC3 \cite{guo2023close}; arXiv papers, PeerRead reviews, Reddit, wikiHow manuals, and Wikipedia in M4 \cite{wang2023m4}; news articles in  MULTITuDE \cite{macko2023multitude}; and MGTBench \cite{he2023mgtbench} that covers short Q\&A from NarrativeQA \cite{kovcisky2018narrativeqa}, SQuAD1.0 \cite{rajpurkar2016squad} and TruthfulQA \cite{lin2022truthfulqa}. %Refer to Appendix \ref{apdx:sotadata} for details about these datasets. 


We evaluate \checkgpt~with three experiments: (1) directly validate \checkgpt~in without any fine-tuning, (2) fine-tuning the last layer of the classification head with 150 samples, and (3) fine-tuning the whole classification head with the entire training set. We also compare \checkgpt~with fine-tuning the entire language models as reported in these papers. %We use 150 pairs of examples for fine-tuning the last layer and the whole training set for fine-tuning the whole classification head. 
As shown in Table~\ref{tab:otherdataset}, \checkgpt~reaches an F1-score of >0.95 for 9 out of the 15 domains in direct validations without finetuning, and reaches >0.9 for two more domains. Unsatisfactory performance are shown on wikiHow and the short Q\&A in MGTBench. Unlike all the writing tasks, the text in wikiHow is highly informal with many imperatives as tips or advice. For the MGTBench, most of the answers consist of a single sentence, and many of them even come with one or two words. For these four domains, the gaps are too large for \checkgpt~to transfer effectively. %We will have a closer look at the linguistic and semantic factors influencing \checkgpt's transferability in Section~\ref{dis:insights}. 
Notably, the fully-tuned \checkgpt~outperforms fine-tuned language models in almost all the domains except M4-Wikipedia, where \checkgpt~is 0.012 lower than RoBERTa. Note full tuning of \checkgpt~takes approximately 120s per epoch, which is considerably less expensive than tuning RoBERTa (1049s per epoch) or DistillBERT (548s per epoch). 

\begin{table}[t]
	\caption{F1-score of evaluating \checkgpt~on SOTA datasets in different domains. Val.: Direct Validation. FT-L: Fine-tuning the last layer. FT-A: Fine-tuning all the layers in the \checkgpt~classifier. All SOTA detectors were trained/tuned with data in the target domain.}\label{tab:otherdataset}
    \setlength{\tabcolsep}{0.39em}
    \vspace{-3mm}
    {
	\begin{tabular}{c|ccc|cc}
 \hline
   \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{\checkgpt} & \multicolumn{2}{c}{SOTA} \\ \cline{2-6}
   & Val. & FT-L & FT-A & Model & F1-score \\\hline
     ArguGPT-WECCL & 1.000 & 1.000 & 1.000 & RoBERTa & 0.994 \\ \hline
     % ArguGPT-CLEC & 0.985 & 0.987 & 1.000 & RoBERTa & - \\
     HC3-Finance & 0.957 & 0.971 & 0.998 & RoBERTa & 0.993 \\
     HC3-Medicine & 0.985 & 0.985 & 0.998 & RoBERTa & 0.995 \\ 
     HC3-OpenQA & 0.936 & 0.948 & 0.999 & RoBERTa & 0.986 \\
     HC3-Reddit & 0.965 & 0.973 & 1.000 & RoBERTa & 1.000 \\
     HC3-Wiki & 0.945 & 0.971 & 0.991 & - & - \\ \hline
     M4-arXiv & 0.995 & 0.999 & 1.000 & RoBERTa & 1.000 \\
     M4-PeerRead & 0.962 & 0.968 & 1.000 & RoBERTa & 0.961 \\
     M4-Reddit & 0.968 & 0.986 & 0.999 & RoBERTa & 0.907 \\
     M4-wikiHow & 0.767 & 0.899 & 0.998 & RoBERTa & 0.997 \\
     M4-Wiki & 0.964 & 0.983 & 0.996 & RoBERTa & 0.997 \\ \hline
     MULTITuDE & 0.951 & 0.956 & 0.989 & RoBERTa & 0.984 \\ \hline
     MGTBench-N & 0.398 & 0.938 & 1.000 & DistillBERT & 0.948 \\
     MGTBench-S & 0.407 & 0.949 & 1.000 & DistillBERT & 0.989 \\
     MGTBench-T & 0.817 & 0.919 & 1.000 & DistillBERT & 1.000 \\
        \hline
        \end{tabular}\vspace{-3mm}}
\end{table}


% Unifiedclassifierfortesting
\begin{table}[t]
	\caption{TPR and TNR (in \%) in new domains.}\label{tab:otherdataset}
    \setlength{\tabcolsep}{0.5em}
    \vspace{-3mm}
    {
	\begin{tabular}{c|ccc|ccc}
 \hline
      \multirow{2}{*}{} & \multicolumn{3}{c|}{w/o fine-tuning} &\multicolumn{3}{c}{w/ fine-tuning}  \\
		\cline{2-7}
        & Task 1 & Task 2 & Task 3 & Task 1 & Task 2 & Task 3 \\\hline
          % \multicolumn{7}{c}{From top to bottom: Wiki, Essay-C, Essay-P, BBC} \\\hline
          \multicolumn{7}{c}{(b) Wiki} \\\hline
         TPR & 100.0 & 99.86 & 98.13 & 99.86 & 98.76 & 94.08 \\
         TNR &  81.13 & 96.50 & 81.13 & 99.23 & 99.54 & 93.85 \\\hline
        \multicolumn{7}{c}{(b) Essay-C} \\\hline
         TPR & 91.09 & 97.13 & 86.82 & 100.0 & 100.0 & 100.0 \\
         TNR & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\\hline
        \multicolumn{7}{c}{(c) Essay-P} \\\hline
         TPR & 83.36 & 68.82 & 79.09 & 99.82 & 99.82 & 99.82 \\
         TNR & 99.92 & 99.77 & 99.92 & 99.69 & 98.75 & 99.37 \\\hline
        \multicolumn{7}{c}{(d) BBC News} \\\hline
         TPR & 100.0 & 99.43 & 90.72 & 100.0 & 99.57 & 97.50 \\
         TNR & 99.86 & 99.93 & 99.86 & 100.0 & 99.86 & 98.79 \\\hline
        \end{tabular}\vspace{-3mm}}
\end{table}

%Does \checkgpt~rely on any ad-hoc patterns that are temporary during a specific period?

\subsection{\checkgpt~Performance Over Time}\label{subsec:transfertovertime}
{
Since its first release, OpenAI has made several major updates to ChatGPT throughout 2023. Hence, we ask the question: \textit{Will \checkgpt~remain effective over time?} We evaluate \checkgpt on ChatLog-HC3 \cite{tu2023chatlog}, which consists of ChaGPT-generated answers for the same questions collected every month starting from 03/2023. In this experiment, we pre-train \checkgpt~with GPABenchmark v1, which was collected before March 2023. As shown in Figure~\ref{fig:chatlog}, \checkgpt's performance has stayed high over the past ten months. Additionally, we have the following observations:

%\begin{itemize}[noitemsep, topsep=1mm, left=0pt]
\noindent$\bullet~$ While we only train/tune \checkgpt~with data prior to 03/2023, it yields stable performance over 10 months. Moreover, \checkgpt's accuracy significantly increased for all the domains on 06/2023. A possible explanation is that an update may have introduced more consistent writing styles and stronger patterns to ChatGPT.

%\noindent$\bullet~$ For Wikipedia, \checkgpt's performance after fine-tuning and even training from scratch is worse than the direct validations. This indicates that \checkgpt~trained on GPABench2 captures the generic and inherent patterns of ChatGPT writing, which contributes more to detection than the domain-specific and/or lexical features in Wikipedia.

\noindent$\bullet~$ \checkgpt~performs worse on OpenQA compared to the original HC3 collected in 12/2022 (Table~\ref{tab:otherdataset}). In a closer look, we find that ChatGPT generated significantly shorter answers in ChatLog. The average length was 133 tokens for HC3-OpenQA but 71 tokens for ChatLog in 03/2023. However, ChatGPT started to generate longer answers later in 2023, with an average length of 98 tokens in December, and the performance of \checkgpt~increases accordingly.

\begin{figure}[!t]
\centering
\includegraphics[width=0.98\columnwidth]{CheckGPT/img/chatlog1.png}\vspace{-3mm}
\caption{TPR on ChatLog-HC3 with direct validation, fine-tuning, and full re-train.}\vspace{-2mm}
\label{fig:chatlog} \vspace{-2mm}
\end{figure}


}

\subsection{Transferability to New LLMs}\label{subsec:transfertonewmodel}

%OpenAI launched GPT-4 on March 14, 2023, while Google released its LLM-based chatbot, Bard, a week later. Bard only provides access through the web interface with high rate limits. Hence, we tested Bard in small-scale experiments. 
{
\noindent \textbf{\em GPT-4.} 
% We invoke Bard and GPT-4 with the same prompts in Sec. \ref{sec:subsecgpabenchmark} to generate LLM-WRI, LLM-CPL, and LLM-POL abstracts for 100 and 2000 random samples, respectively (small sample size due to a lack of API (Bard) and strict rate limits). We use the unified classifiers to evaluate all the samples and show the TPRs in Table \ref{tab:bard}. \checkgpt~achieves >96\% TPR in 5 experiments. The TPR for Bard-polished text is relatively low. Further investigation shows that Bard makes minimal changes (e.g., copy editing a few words) for some samples. Therefore, these misclassifications appear reasonable. 
We invoke GPT-4, which is the most up-to-date and powerful member of GPT models, with the same prompts in Sec. \ref{sec:subsecgpabenchmark} to generate GPT-WRI, GPT-CPL, and GPT-POL abstracts for  2000 random samples, respectively (small sample size due to strict rate limits). We use the unified classifiers to evaluate all the samples, and \checkgpt~achieves >96\% TPR in all three experiments (99.95\%, 96.90\%, and 96.15\%, respectively).

\noindent \textbf{\em Non-GPT LLMs.} 
Other LLMs might adopt unique model architectures, training datasets, and training methodologies, which may differ significantly from ChatGPT. In this paper, we do not claim or expect the transferability of \checkgpt~to non-GPT LLMs. %Actually, we don't expect \checkgpt~trained on GPT content to be universal to all kinds of LLM patterns. However, \checkgpt~is applicable to AIGC detection of any other LLM. 
Nevertheless, we still apply \checkgpt~(without tuning) to the content generated by 11 non-GPT LLMs: M4 \cite{wang2023m4}, MULTITuDE \cite{macko2023multitude}, and MGTBench \cite{he2023mgtbench}. As shown in Figure~\ref{tab:otherllms}, \checkgpt~is highly adaptable to content generated by all the LLMs. Note that the F1-scores for models other than ChatGPT in M4 are not reported in \cite{wang2023m4}.

% \begin{table}[t]
% 	\caption{F1-score of \checkgpt's performance with non-GPT LLMs. SOTA: the performance of fine-tuned language models.}\label{tab:otherllms}
%     \setlength{\tabcolsep}{0.3em}
%     \vspace{-3mm}
%     \centering
%     {\small 
% 	\begin{tabular}{c|c|cc|cc}
%  \hline
%    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Other LLMs} & \multicolumn{2}{c|}{\checkgpt} & \multicolumn{2}{c}{SOTA} \\ \cline{3-6}
%    && Min. & Avg. & Min. & Avg. \\\hline 
%      M4-arXiv & \multirow{3}{*}{\parbox{3cm}{\centering BloomZ, Cohere, Dolly, Flant-T5}} & 0.998 & 0.999 & - & -\\
%      M4-PeerRead & & 0.996 & 0.999 & - & -\\
%      M4-Reddit & & 0.984 & 0.996  & - & -  \\ \cline{2-2}
%      M4-wikiHow & \multirow{2}{*}{BloomZ, Cohere, Dolly} & 0.988 & 0.995   & - & -  \\
%      M4-Wiki & & 0.978 & 0.989   & - & - \\ \hline
%      \multirow{2}{*}{MULTITuDE} & Alpaca, LLaMA, OPT, 
%      & \multirow{2}{*}{0.937}& \multirow{2}{*}{0.965}& \multirow{2}{*}{0.883}& \multirow{2}{*}{0.941}
%      \\ 
%      & OPT-IML, Vicuna & & & & \\\hline
%      MGTBench-N & \multirow{3}{*}{ChatGLM, Dolly, StableLM} & 1.000 & 1.000 &  0.875 & 0.928  \\
%      MGTBench-S &  & 1.000 & 1.000 & 0.939 & 0.965 \\
%      MGTBench-T &  & 1.000 & 1.000 & 0.966 & 0.988   \\
%        \hline 
%         \end{tabular}\vspace{-3mm}}
% \end{table}

\begin{table}[t]
	\caption{Performance (F1-score) of \checkgpt~on non-GPT LLMs. SOTA: the performance of fine-tuned language models.}\label{tab:otherllms}
    \setlength{\tabcolsep}{0.15em}
    \vspace{-3mm}
    \centering
    {\small 
	\begin{tabular}{c|c|cc|cc|cc}
 \hline
   \multirow{2}{*}{Dataset} & \multirow{2}{*}{Other LLMs} & \multicolumn{2}{c|}{FT-L} & \multicolumn{2}{c|}{FT-A} & \multicolumn{2}{c}{SOTA} \\ \cline{3-6}
   & & Min. & Avg.& Min. & Avg. & Min. & Avg. \\\hline 
     M4-arXiv & \multirow{3}{*}{\parbox{2.5cm}{\centering BloomZ, Cohere, Dolly, Flant-T5/Llama}} & 0.903 & 0.927 & 0.998 & 0.999 & - & -\\
     M4-PeerRead & & 0.820 & 0.868 & 0.996 & 0.999 & - & -\\
     M4-Reddit & & 0.872 & 0.987 & 0.984 & 0.996  & - & -  \\ \cline{2-2}
     M4-wikiHow & \multirow{2}{*}{\parbox{2.5cm}{\centering BloomZ, Cohere, Dolly}} & 0.834 & 0.915 & 0.988 & 0.995   & - & -  \\
     M4-Wiki & & 0.798 & 0.847 & 0.978 & 0.989   & - & - \\ \hline
     \multirow{2}{*}{MULTITuDE} & Alpaca, LLaMA, OPT, 
     & \multirow{2}{*}{0.656} & \multirow{2}{*}{0.758} & \multirow{2}{*}{0.937}& \multirow{2}{*}{0.965}& \multirow{2}{*}{0.883}& \multirow{2}{*}{0.941}
     \\ 
     & OPT-IML, Vicuna & & & & \\\hline
     MGTBench-N & \multirow{3}{*}{\parbox{2.5cm}{\centering ChatGLM, Dolly, StableLM}} & 0.909 & 0.934 & 1.000 & 1.000 &  0.875 & 0.928  \\
     MGTBench-S &  & 0.908 & 0.919 & 1.000 & 1.000 & 0.939 & 0.965 \\
     MGTBench-T &  & 0.920 & 0.956 & 1.000 & 1.000 & 0.966 & 0.988   \\
       \hline 
        \end{tabular}\vspace{-3mm}}
\end{table}


}


% \begin{table}[t]
% 	\caption{\checkgpt's TPR (in \%) for Bard and GPT-4.}\label{tab:bard}
%     \setlength{\tabcolsep}{0.15em}
%     \vspace{-3mm}
%     \centering
%     {\small
% 	\begin{tabular}{c|ccc|p{2mm}c|ccc}
%          %\multicolumn{3}{c|}{Bard (Tasks 1, 2, 3)} &\multicolumn{3}{c}{GPT-4}  \\\hline
% 		%\hline
%        \multirow{2}{*}{Bard} & Task 1 & Task 2 & Task 3 & & \multirow{2}{*}{GPT-4} & Task 1 & Task 2 & Task 3 \\\cline{2-4}\cline{7-9}
%         & 99.00 & 96.00 & 82.00 & & & 99.95 & 96.90 & 96.15\\
%         % 50/50 53/53 44/51
%         % 80/81 80/83 66/81
%         \end{tabular}\vspace{-4mm}}
% \end{table}

\subsection{Advanced Prompt Engineering}\label{sec:prompteng}

% \subsection{Selection of Disciplines and Tasks}
% As we mentioned in Sec~\ref{sec:subsecgpabenchmark}, we select three different tasks and disciplines based on their different nature. Actually, we expect a series of characteristics of these tasks and disciplines. The experiments also validate many of our expectations. Actually, we have the following observations considering the difference:

% \begin{itemize}[noitemsep, topsep=1mm, left=0pt]
% \item \textbf{}
% \end{itemize}


% \subsection{Prompt Engineering} \label{sec:prompteng}

% Prompts are used to provide instructions to conversational LLMs to customize/refine their responses. 
%Research efforts on prompt engineering aim to guide or improve the design of ChatGPT prompts \cite{white2023prompt,ekin2023prompt}. We select six approaches that are widely adopted in the community: (1) Zero-shot Chain-of-Thought Prompting (ZC, \citealp{zeroshot}) enforces step-by-step reasoning with specific trigger phrases like ``Let's think step by step.'' (2) Automatic Prompt Engineer (APE, \citealp{ape}) automates the creation and selection of prompts using iterative optimization. (3) Self-critique Prompting (SCP, \citealp{critique}) employs GPT to evaluate its own responses and provide feedback. (4) Few-shot Prompting (FSP, \citealp{fewshot}) conditions the model using examples or demonstrations. (5) Least-to-Most Prompting (LMP, \citealp{least}) parses a problem into simpler subproblems. (6) Generated Knowledge Prompting (GKP, \citealp{generated}) starts the prompt with relevant information generation. We also adopt four prompt refinement methods: (1) Prompt Perfect (PP, \citealp{promptperfect}). (2) GPT-generated Prompts (GP, \citealp{Creator}). (3) Meta Prompts (MP, \citealp{metaprompt}). (4) Instruction Induction (II, \citealp{honovich2022instruction}, not for Task 3). We use each method to write, complete, and polish 5,000 abstracts from each discipline (please refer to Appendix~\ref{apdx:otherprompt} for details).% in GPABenchmark: 

% \noindent\textbf{Prompt 1}: %\cite{jaiswal2023prompts}: 
% \textit{Rewrite the following abstract of a research paper in first-person, clear, and academic language} 

% %\checkgpt's detection accuracy: 90.07\%.

% \noindent\textbf{Prompt 2}: %\cite{PlexPt2023prompt}: 
% \textit{Please act as an expert paper editor and revise the abstract section of the paper from the perspective of a paper reviewer to make it more fluent and elegant. Here are the specific requirements:} [See Appendix~\ref{apdx:prompt2} for full prompt]

% %\checkgpt's detection accuracy:  93.57\%

% % \noindent\textbf{Prompt 3}\cite{nigh2023prompt}: \textit{Refine the existing abstract of a research paper by using academic language to make it more clear and fluent.}

% % \checkgpt's detection accuracy: 86.15\%

% \noindent\textbf{Prompt 3}: %\cite{amiri2023prompt}: 
% \textit{Write a polished and refined version of the following abstract of a research paper to improve its overall quality and readability.}

% %\checkgpt's detection accuracy: 95.15\%

% \noindent\textbf{Prompt 4}: %\cite{Akın2023prompt}: 
% \textit{I want you to act as an academic researcher. You will be responsible for rewriting the abstract of a research paper for clarity. Here is the original abstract of the paper:}

% %\checkgpt's detection accuracy: 97.35\%

% \noindent\textbf{Prompt 5}: %\cite{Akın2023prompt}: 
% \textit{I want you to act as an academic paper writer. You will be responsible for rewriting a paper abstract. Your task is to improve the writing and clarity of the abstract. Here is the original abstract of the paper: }

%\checkgpt's detection accuracy: 91.78\%

% \noindent\textbf{Prompt 5}\cite{Akın2023prompt}: \textit{I want you to act as an academician. You will be responsible for rewriting the abstract of a research paper for clarity. Here is the original abstract of the paper:}

% \checkgpt's detection accuracy: 88.33\%
As presented in Section \ref{sec:subsecgpabenchmark}, GPABench2 contains 435K additional testing samples using advanced prompt engineering. We evaluate the new dataset with task-specific, discipline-specific, and cross-prompt classifiers. As shown in Table \ref{tab:moreprompt}, \checkgpt's TPRs are consistently high. Moderate decreases are only noticed in LMP, SCP, GKP, MP, and II for Task 2, and LMP for Task 3. However, when a prompt-specific (P1) model is used for the new data, the average TPR decreases by 0.85\%, and the maximum decrease is 8.2\% (detailed in Appendix~\ref{apdx:promptsingle}). This suggests the robustness of the cross-promote models, i.e., the models learned GPT-specific features that are transferable,  instead of prompt-specific bias. 

%and report the TPRs in Table \ref{tab:moreprompt}. Specifically, we have the following observations: (1) \checkgpt's accuracy experiences a minor decrease but consistently exceeds 97\%, except II. (2) For Task 1, the choice of prompting methods doesn't affect accuracy. (3) For Task 2, LMP, SCP, and GKP moderately impact \checkgpt, while MP and II have a significant effect. (4) For Task 3, only LMP has a negative impact.

% \begin{table}[t]
% 	\caption{\checkgpt's TPR on different prompts.}\label{tab:promptengineering}
%     \setlength{\tabcolsep}{0.4em}
%     \centering
%     \vspace{-2mm}
%     {\small
% 	\begin{tabular}{cccccc}
% \hline
% \multicolumn{6}{c}{CS} \\\hline
% & ZC & APE & SCP & FSP & LMP \\
% \hline
% Task 1  & 100.0 & 100.0 &  99.95& 100.0 & 99.94 \\
% Task 2  & 99.38 & 99.11 &  99.15& 99.68 & 98.60 \\
% Task 3  & 99.79 & 99.47 &  99.64& 99.45 & 99.01 \\
% \hline
%  & GKP & PP & GP & MP & II \\
% \hline
% Task 1  & 99.96 & 100.0 & 99.64 & 99.96 & 100.0\\
% Task 2  & 98.50 & 99.66 & 99.78 & 97.78 & 99.21\\
% Task 3  & 99.78 & 99.84 & 99.19 & 99.58 & -\\
% \hline
% \hline
% \multicolumn{6}{c}{PHX} \\\hline
%  & ZC & APE & SCP & FSP & LMP \\
% \hline
% Task 1  & 100.0 & 100.0 &  99.94& 99.98 & 99.98 \\
% Task 2  & 98.91 & 99.21 &  98.43& 99.61 & 98.97 \\
% Task 3  & 99.84 & 99.26 &  99.81& 99.24 & 98.99 \\
% \hline
%  & GKP & PP & GP & MP & II \\
% \hline
% Task 1  & 99.98 & 100.0 & 99.59 & 99.98 & 99.98\\
% Task 2  & 98.62 & 99.90 & 99.59 & 97.75 & 98.53\\
% Task 3  & 99.73 & 99.88 & 99.48 & 99.65 & -\\
% \hline
% \hline
% \multicolumn{6}{c}{HSS} \\\hline
% & ZC & APE & SCP & FSP & LMP \\
% \hline
% Task 1  & 100.0 & 99.96 & 99.98 & 99.92 & 99.94\\
% Task 2  & 99.21 & 99.21 & 98.67 & 99.44 & 98.85\\
% Task 3  & 99.79 & 99.27 & 99.73 & 99.54 & 98.89\\
% \hline
%  & GKP & PP & GP & MP & II \\
% \hline
% Task 1  & 100.0 & 99.98 & 99.83 & 99.98 & 99.96\\
% Task 2  & 98.70 & 99.54 & 99.67 & 97.97 & 99.00\\
% Task 3  & 99.80 & 99.83 & 99.33 & 99.73 & - \\
% \hline

% \end{tabular}}
% \end{table}

\begin{table}[t]
	\caption{TPR (in \%) for advanced prompts.}\label{tab:moreprompt}
    \setlength{\tabcolsep}{0.39em}
    \centering
    \vspace{-3mm}
    {\small
	\begin{tabular}{c|ccc|ccc|ccc}
 \hline
        & \multicolumn{3}{c}{T1. GPT-WRI} &\multicolumn{3}{c}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\ \cline{2-10}
         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
         ZC & 100.0 & 100.0 & 100.0 & 99.38 & 98.91 & 99.21 & 99.79 & 99.84 & 99.79\\
         APE & 100.0 & 100.0 & 99.96 & 99.11 & 99.21 & 99.21 & 99.47 & 99.26 & 99.27\\
         SCP  & 99.95 & 99.94 & 99.98 & 99.15 & 98.43 & 98.67 & 99.64 & 99.81 & 99.73\\
         FSP & 100.0 & 99.98 & 99.92 & 99.68 & 99.61 & 99.44 & 99.45 & 99.24 & 99.54\\
         LMP & 99.94 & 99.98 & 99.94 & 98.60 & 98.97 & 98.85 & 99.01 & 98.99 & 98.89\\
         GKP & 99.96 & 99.98 & 100.0 & 98.50 & 98.62 & 98.70 & 99.78 & 99.73 & 99.80\\
         PP & 100.0 & 100.0 & 99.98 & 99.66 & 99.90 & 99.54 & 99.84 & 99.88 & 99.83\\
         GP  & 99.64 & 99.59 & 99.83 & 99.78 & 99.59 & 99.67 & 99.19 & 99.48 & 99.33\\
         MP & 99.96 & 99.98 & 99.98 & 97.78 & 97.75 & 97.97 & 99.58 & 99.65 & 99.73\\
         II & 100.0 & 99.98 & 99.96 & 99.21 & 98.53 & 99.00 & - & - & -\\ \hline
\end{tabular}}\vspace{0mm}
\end{table}

\subsection{Discussions on \checkgpt's Transferability}\label{dis:insights}\label{sec:discussion}

With all the task-, prompt-, model-, and domain-transferability experiments, we raise the critical questions: \textit{What makes \checkgpt~trained on GPABench2 (non-)transferable to other domains}? \textit{How can GPABench2 contribute to general-purpose GPT-text detection}? To investigate this, we again adopt the NELA feature to measure the domain gaps between GPABench2 and all the 39 target domains in the transferability experiments, e.g., Wiki, ASAP Essays, BBC News, etc. We %calculate the centroids of the NELA feature vectors in each domain and 
examine the correlation of each feature with CheckGPT's transferability, i.e., the performance of \checkgpt~in validations without fine-tuning. We set a threshold at 0.5 on Spearman's Rank Correlation Coefficient. Eventually, we obtain the positive and negative factors influencing the transferability of \checkgpt, as shown in Figure~\ref{fig:spearman}. The top six positive features are (from high to low): Fairness Virtue, Readability (Coleman-Liau Index, average word length, LIX Readability, and Smog Index), adjectives, plural nouns, gerunds. The top two negative factors are quotes and particles. 

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{CheckGPT/img/spearman.png} \vspace{-9mm}
\caption{Correlations between domain-specific features and \checkgpt's transferability.} %\vspace{-3mm}
\label{fig:spearman}\vspace{-3mm}
\end{figure}

Based on the positive factors, we conclude that \textit{\checkgpt~will transfer better to objective, complex, detailed, narrative, or journalistic writing. } Firstly, the fairness virtue indicates an objective tone, while higher readability indicates longer and more complex sentences and word usage. Secondly, descriptive language plays an important role in writing styles with more adjectives. Adjectives add details and expressiveness to the writing by qualifying nouns and pronouns. More adjectives improve the clarity and vividness of the text, indicating creative or detailed writing. Thirdly, writing styles that frequently use plural nouns typically involve discussion of general concepts, discovery, groups, or disciplines rather than focusing on individual or specific instances. They usually serve a technical, scientific, analytical, or political purpose. Lastly, as we have shown in Section~\ref{subsec:baseline}, ChatGPT favors gerunds and \checkgpt~will transfer to descriptive or narrative writing with a sense of continuous actions and processes.

Similarly, based on the negative factors, we conclude that \textit{\checkgpt~will possibly show less transferability to informal writing and conversations, } as particles and quotes will appear more frequently in these writing styles.



\subsection{Use of ChatGPT in arXiv 
Papers} \label{sec:arxivstudy}
%The usage of LLMs is growing rapidly. 

%ChatGPT reached 1.8 billion visits in the month of April 2023. Microsoft also reported the new Bing AI with online GPT-4 has been used more than 500 million times in twenty days. 

%With the popularity of LLMs/ChatGPT, 
Finally, we ask ``\textit{How many authors are using ChatGPT to write/polish their research papers}?'' We collect all the arXiv abstracts in CS from January 2016 to December 2023 ($\sim$450k samples, excluding those in GPABench2). We evaluate each abstract with the unified cross-task cross-prompt cross-disciplinary classifier and show the monthly average positive rates in Figure \ref{fig:distlength}. There is a significant increase in ChatGPT usage with a peak of 26.1\% in December 2023. The average positive rates before, between, and after the releases of GPT-3 and ChatGPT are 1.12\%, 1.78\%, and 7.83\%, respectively. The exponential growth started in December 2022, right after ChatGPT's release on 11/30/2022. Our model also annotates 0.23$\sim$1.66\% of the abstracts posted before GPT3 as GPT-GEN, which may be explained by \checkgpt's 1\% FPR, while LLMs like GPT-2 might also be used by the early adopters.

% Finally, we would like to emphasize that the human-written abstracts in GPABenchmark were collected from papers published on or before 2021, when access to GPT-3 was restricted to invited testers. Hence, we are confident that the labels in the GPABenchmark dataset are reliable.

%test it against our models trained for three tasks. According to our results, we notice that the ratio of the abstracts labeled as "GPT-generated" increased by 8x over the past nine months. The launch of the public version of ChatGPT is in December 2022, which is in coincidence with a considerable jump in the positive ratio according to our models. Especially during the last three months, the positive cases significantly flourish, reaching a peak of 12.54\% in May 2023. The results are shown in Fig~\ref{fig:distlength}.

% However, it is important to acknowledge that the ground truth labels of our real-world data, which can be used for validation of our results, are not publicly available. Actually, the ground truth should be impractical, if not likely, to obtain. Despite this, the results of our study provide indicative observations. According to our model, the ratio of the abstracts labeled as "GPT-generated" has been consistently and relatively low until the release of ChatGPT, but it started to escalate exponentially ever since the "Big Bang". 

\begin{figure}[!t]
\centering
\includegraphics[trim={0 0 0 8mm},clip, width=0.96\columnwidth]{CheckGPT/img/byyear_plot_task13_ccs.png}\vspace{-4mm}
\caption{Detecting ChatGPT usage in arXiv papers.}
\label{fig:distlength}\vspace{-4mm}
\end{figure}
% [14.018, 13.546, 8.749, 6.645, 5.192, 4.452, 3.559, 3.778, 3.030, 2.985, 2.822, 2.838]

%It is also worth noting that the samples in arXiv we used for our training are all published before or in 2021. Thus, the model error as a result of domain shift cannot account for all the increases. Moreover, it cannot explain the difference between the ones before and after the public release of ChatGPT. The positive rates for the first six months are slightly larger when compared with our results in Sec~\ref{sec:baselineperf}. This might be due to two reasons: Firstly, users may have employed other similar LLMs, such as GPT-3, for academic writing before the accessibility of ChatGPT. Secondly, for our real-world study, we investigate the abstracts across all the disciplines on arXiv, including biology and economics. The changes in disciplines may also account for the inflated ratio.

%Beyond the real-world implications, there is also another noteworthy finding according to our results. Given the preassumption that a significant portion of the positive cases, if not most of them, have been written with the help of ChatGPT, \checkgpt~demonstrates scalability considering the prompts. The real-world users will use their own prompts designed by themselves in a case-by-case situation. Even when the prompts used by people are black-box and inaccessible, \checkgpt~is still insightful and robust for effective detection.

% \subsection{Linguistics and Comparison}

% \subsection{Ablation Study}
% % Random Ablation
% Crossover

\subsection{Robustness against Sanitized GPT Output} \label{sec:robustness}
{
We consider the scenario where the user (attacker) sanitizes the raw output from ChatGPT to make it more human-like, in an attempt to escape \checkgpt. We discuss and implement four attacks: 

\noindent\textbf{\em Automatic Rephrasing.} The attacker prompts ChatGPT to rephrase its answers twice. In each prompt, ChatGPT is asked to rephrase its output to make it ``more like human-written.''

\noindent\textbf{\em Mixed Human/GPT Writing (The Mixing Attack).} The attacker substitutes some of the ChatGPT-generated text with human-written text to confuse the detector. In particular, ChatGPT-written abstracts are usually 6-8 sentences long, where the first and last sentences are more generic and less technical. We substitute \textit{each} of the top 3 and last 3 sentences with the corresponding sentence from the HUM abstract. We further attempt to substitute two sentences (top 2 or last 2) from GPT-GEN abstracts. In the end, each attack sample is a hybrid text with GPT-GEN and HUM content.

\noindent\textbf{\em Copyediting.} We make a strong attack assumption that the attacker knows the vocabulary distribution of GPT- and HUM-generated text, and sanitizes GPT text accordingly. To mimic this attack, we examine word and bi-gram distribution in HUM- and GPT-generated abstracts in GBABench2, and identify the words and phrases with the largest frequency discrepancy. i.e., words that are popular in GPT-GEN but rarely used in HUM-WRI. We drop the attributives, and substitute the other words/bigrams that are popular in ChatGPT text with synonyms that are heavily used by humans. Based on the attackers' knowledge and costs, we define three attack levels: Top-3, Top-5, and Top-10. We extract the Top-N words and phrases in each discipline, task, and prompt and combine them in one set. Eventually, there are 76 items in the Top-10 set and 52 items in the Top-3 set. Some examples of substitutions in all three levels include removing or replacing ``this paper'', ``the paper'', ``this study'', ``in this paper'', ``in this study'', ``additionally'', ``furthermore'', etc. Please see Appendix~\ref{apdx:ceaattack} for the detailed vocabulary and substitutions. 

\noindent\textbf{\em Prompt Engineering.} Same as the Copyediting Attack, the attacker knows the term distributions of HUM- and GPT-generated texts. The attacker employs prompt engineering to ask ChaGPT to avoid using the words and phrases that are popular in GPT-GEN text.  

We evaluate our cross-prompt cross-discipline cross-task classifier against 10,000 attack samples for each combination of task, discipline, and prompt. The TPRs are shown in Table~\ref{tab:attacks}. We have the following observations:

%\begin{itemize}[noitemsep, topsep=1mm, left=0pt]
\noindent$\bullet~$ \checkgpt's accuracy becomes higher on rephrased text, i.e., nearly 100\% TPR for all the tasks/discipline. It implies that the inherent patterns of ChatGPT get stronger after iterative rewriting.

\noindent$\bullet~$ \checkgpt~is robust when any of the first/last 3 sentences is replaced with a human sentence. Performance for a few tasks dropped to $\sim$75\% when two sentences (about 1/4 to 1/3 of the abstract) are replaced,  while the other tasks still perform >90\%. That is, \checkgpt's detection is not dominated by any single sentence-level indicator. Instead, every sentence contributes to the decision.  


\noindent$\bullet~$ \checkgpt's detection accuracy decreases slightly when the unique terms used by ChatGPT (sometimes referred to as ``artifacts'') are removed or replaced with ``human terms''. However, the average TPR remains at 83.1\% (with a minimum of 70.45\%) after removing/replacing 76 top words and phrases in GPT-GEN text. This implies that \checkgpt~learns and utilizes the lexical features in GPT-generated content, but it does not completely rely on them.

\noindent$\bullet~$ \checkgpt~provides the lowest accuracy with Copyediting Attacks in Task 3. In this polishing task, ChatPGT mostly maintains the structure of the paragraph and the sentences but makes word-level tuning. Therefore: (1) The semantic and structural features of GPT-POL abstracts are very similar to HUM abstracts. And (2) the lexicon features of GPT-POL abstracts are effectively eliminated by the manual Copyediting Attack. Both factors contribute to the low accuracy of \checkgpt~against this attack.  

%This can be explained for two reasons: (1) The nature of Task 3 is to ask ChatGPT to polish the human-written text. Thus, it is well expected that ChatGPT will use as many "advanced" expressions as possible, which are less used by human writers. (2) compared to Task 1 and 2. Thus, \checkgpt~will relies more on lexical features.

\noindent$\bullet~$ \checkgpt's performance stays high against the Prompt Engineering Attacks. This shows that the ChatGPT's habitual patterns persist even under specially crafted instructions, which aligns with our findings in Section~\ref{sec:prompteng}.

In summary, \checkgpt~is highly robust against \textit{post facto} human interventions of ChatGPT-generated content at word/phrase and sentence levels. As we have observed, \checkgpt~employs many ``weak indicators'' from lexicon, structural, and semantic features that are scattered across the entire text snippet to collectively support a classification decision with relatively strong confidence. 

%The subtle ``clues'' are accumulated throughout the whole text.

%\noindent$\bullet~$  Among the three tasks, \checkgpt~is the most sensitive on Task 3 GPT-POL abstracts, especially for CS and HSS. By looking at Mixing and CopyEditing attacks, we find that every word and sentence contributes to \checkgpt's detection. As discussed previously, Task 3 is the most challenging. Thus, the subtle difference between HUM and GPT-POL abstracts is captured by \checkgpt~with multi-faceted features.

%However, as we have discussed in Section~\label{subsec:model}, the goal of this paper is to understand and detect ChatGPT-generated content. Thus, advanced attackers with white-box access to \checkgpt's parameters and those who perform a thorough manual rewriting are out of our scope. 

\begin{table}[t]
	\caption{TPR (in \%) under attacks. CE: Copyediting. PromptEng: Prompt Engineering Attacks. Mixing-F/L: substituting the first/last sentences.}\label{tab:attacks}
    \setlength{\tabcolsep}{0.128em}
    \centering
    \vspace{-1mm}
    {
	\begin{tabular}{c|ccc|ccc|ccc}
 \hline
        & \multicolumn{3}{c}{T1. GPT-WRI} &\multicolumn{3}{c}{T2. GPT-CPL}  &\multicolumn{3}{c}{T3. GPT-POL}\\ \cline{2-10}
         & CS & PHX & HSS & CS & PHX & HSS & CS & PHX & HSS\\\hline
         Rephrasing & 100.0 & 100.0 & 100.0 & 99.99 & 99.98 & 100.0 & 99.99 & 99.97 & 99.95\\ % type3
         Mixing-F1 & 99.98 & 100.0 & 99.93 & 99.52 & 99.54 & 99.33 & 93.10 & 97.31 & 91.52\\ %type5_1
         Mixing-F2 & 99.98 & 100.0 & 99.98 & 99.21 & 99.44 & 99.09 & 95.73 & 98.00 & 95.28\\ %type5_2
         Mixing-F3 & 99.89 & 99.97 & 99.77 & 97.59 & 98.62 & 96.83 & 90.52 & 96.22 & 90.73\\ %type7_5
         Mixing-L3 & 99.96 & 99.97 & 99.85 & 99.02 & 99.54 & 98.57 & 96.71 & 98.18 & 96.79\\ %type7_6
         Mixing-L2 & 99.83 & 100.0 & 99.87 & 98.14 & 99.24 & 98.03 & 94.63 & 98.17 & 94.52\\ %type5_3
         Mixing-L1 & 99.80 & 100.0 & 99.78 & 95.21 & 97.33 & 96.24 & 96.44 & 98.39 & 95.83\\ %type5_4
          Mixing-F12 & 99.77 & 99.97 & 99.31 & 96.90 & 97.63 & 95.62 & 75.78 & 87.55 & 73.02\\
          Mixing-L12 & 
          95.60 & 98.20 & 96.43
          & 78.05 & 85.57 & 82.67
          & 75.68 & 94.14 & 85.75\\
         CE-Top3 & 96.55 & 98.47 & 92.79 & 93.06 & 95.35 & 91.88 & 83.77 & 91.88 & 85.85\\ %type10
         CE-Top5  & 92.92 & 96.47 & 88.83 & 89.06 & 92.25 & 87.35 & 78.36  & 89.84 & 81.17\\ %type9
         CE-Top10 & 89.27  & 92.62  & 82.02 & 85.75 & 88.52  & 82.54 & 70.45 & 84.20 & 72.56\\ %type11
         PromptEng & 99.99 & 99.94 & 99.99 & 99.19 & 99.02 & 99.62 & 89.92 & 89.30 & 95.92\\ %type2
         \hline
\end{tabular}}\vspace{-2mm}
\end{table}

%\subsection{Multi-task Classifier} \label{sec:multitask}




==> CheckGPT/tex/intro.tex <==
\section{Introduction}
\label{sec:intro}

The recently debuted Large Language Model (LLM) - ChatGPT has shown an impressive ability to generate sophisticated texts with human-like language style and quality. Concerns have been raised that the LLM-generated content (LLM-content) can be misused to abuse the trust systems we have, e.g., in cheating and plagiarism \cite{stokel2022ai,khalil2023will}, or in phishing and romance scams \cite{roy2023generating,grbic2023social}. While many academic institutes and publishers have announced policies on the usage of LLM content, it is hard to enforce such policies unless we have a tool to accurately detect LLM content.

LLM-content detection can be challenging due to the unique characters of LLM/ChatGPT: (1) like a human conversationalist, the output of LLM has a relevant, organized response with a low level of grammar errors; (2) the sampling mechanism of LLM output ensures that the choice of words is stochastic, therefore, the responses are distinct even with multiple repeated inquiries; and (3) the misuse of LLM-content can be stealthy since users can invoke ChatGPT to polish human writing. Facing these challenges, existing LLM detectors perform deficiently, especially in detecting GPT-polished text (Sec. \ref{sec:comparison}). Some experiences in identifying LLM-content have been reported in the literature, e.g., \citet{guo2023close} and \citet{liu2023argugpt} noted that ChatGPT output tends to be more objective, formal, focused, and fluent than human-content. However, a holistic investigation of the distinguishability of LLM-Content is still missing. 

To this end, in this paper, we first identify three typical cases of using or abusing ChatGPT in academic writing: {\em composing}, {\em completing}, and {\em polishing}. We pick three representative disciplines for investigation: \textit{computer science} for technical/engineering writing, \textit{physics} for science writing, and \textit{humanities and social sciences} for liberal arts writing. To address a range of complex real-world scenarios, we used four different prompt patterns for each task across each discipline and collected a dataset, \textit{GPABench2}, with 2.8 million human-written and ChatGPT-generated academic abstracts. %, for the nine combinations of tasks and disciplines. 
% To the best of our knowledge, GPABenchmark is the most comprehensive and publicly available ChatGPT-generated dataset of academic writing by far.

%To validate the difficulty of detecting LLM-content in academic writing, we carry out both human- and algorithm-evaluation. 
Next, we conducted an extensive field study with human evaluators to assess if they can distinguish LLM content accurately provided with a mixture of true and false samples. The cohort of 155 evaluators consisting of university faculty, researchers, and graduate students, proves that the recognition of LLM-content is difficult for visual inspection based on language appearance, with or without individual experiences of writing research articles. A second cohort of 87 evaluators were provided with ground truth data as references: pairs of human-written and GPT-generated abstracts. While their capacities to identify human- and GPT-generated text were improved, the accuracy is still too low for reliable detection. In addition, we test 10+ state-of-the-art online or open-source detectors on GPABench2, e.g., GPTZero, and show that they demonstrate modest to poor performance, except for the language-model-based detectors, like BERT and RoBERTa, which archives significantly better result but requires excessive training efforts. 

Last, we develop and evaluate a language-model-based detection framework, named \checkgpt, to explore the feasibility of building automated tools for LLM-content detection in a niche area. \checkgpt~has the following advantages: (1) it is a black-box solution that leverages deep learning frameworks to achieve a high accuracy compared to human and state-of-the-art (SOTA) LLM-content detectors. 
(2) \checkgpt~adopts a model-agnostic setting that it can be treated as a plugin to most pre-trained language models (e.g., BERT), as a result, the number of parameters to be trained can be largely reduced. (3) Due to its ability to learn generalized semantic patterns of LLM-content, \checkgpt~shows a strong potential for domain transfer that only requires minimum fine-tuning efforts. %, our model can quickly pick up the ability to detect LLM-content in new disciplines/domains. 
Finally, we conduct comprehensive experiments to demonstrate \checkgpt's design goals and strengths: its performance on the GPABench2 dataset, its transferability to new domains, new models, and new prompts, and its robustness against continuous updates of ChatGPT and against human-modified GPT writing. 


In summary, our main contributions are:

\begin{itemize}[itemsep=0.5pt,topsep=0.5pt,leftmargin=*]
\item We present %a GPT-generated academic writing dataset - 
GPABench2, a cross-disciplinary corpus consisting of human-written, GPT-written, GPT-completed, and GPT-polished research paper abstracts. GPABench2 has the potential to serve as a cornerstone for benchmarking GPT detectors, and a valuable resource to assist in the design of new detecting methods.
\item We evaluate the SOTA GPT detectors with GPABench2 and present their performance. {Meanwhile, with a user study of 242 participants, we show that human evaluators are unable to distinguish between human-written and GPT-generated academic writing. This incapability persists regardless of experience, knowledge, and reference. }
\item We present \checkgpt, a deep-learning-based and model-agnostic GPT-content detector with validated benefits of affordability, transferability, and Robustness\footnote{We share \checkgpt~at \url{https://anonymous.4open.science/r/CheckGPT-80B2}}.
%representation module and an LSTM-based classification head. 
We demonstrate the outstanding performance ($\sim$99\% average accuracy) of \checkgpt~with extensive experiments.
% \item {\newc We unveil the behavioral patterns of ChatGPT in generating academic writing and analyze how they contribute to CheckGPT's effectiveness and transferability.}
\end{itemize}


\vspace{1mm}\noindent\textbf{{Ethical Considerations.}} The user study in Section \ref{sec:survey} was reviewed and approved by the Human Research Protection Program at the University of [Anonymized]. 
All the research paper abstracts collected in Section \ref{sec:gpabenchmark} are open to the public. We invoked ChatGPT's API (with payment) to collect the GPT-generated abstracts. The GPABench2 dataset and the \checkgpt~tool have been open-sourced. The academic community is actively discussing how AI writing assistance tools may pose challenges to research and education \cite{sallam2023chatgpt,malinka2023educational,anders2023using}. OpenAI also posted their perspectives on the education-related risks and opportunities \cite{openai2023educator}. %In this paper, we provide a detection tool for LLM-Content. 

% The impact of ChatGPT and other AI writing assistance tools on academic integrity is outside of the scope of the paper. 

The rest of the paper is organized as follows: %we introduce the background of LLM and survey the related literature in Section \ref{sec:background}. 
We introduce the GPABench2 dataset and evaluate the open-source and commercial ChatGPT detectors in Section \ref{sec:gpabenchmark}, followed by a user study of ChatGPT-content detection in Section \ref{sec:survey}. We present the technical details of \checkgpt~in Section \ref{sec:checkgpt} and experimental results in Section \ref{sec:exp}. %{\newc Finally, we analyze the prompt engineering, linguistics, and model interpretation in Sections \ref{sec:discussion}}, 
Finally, we survey the related literature in Section \ref{sec:background}, and conclude the paper in Section \ref{sec:conclusion}. 


\iffalse
\begin{itemize}
    \item Introduction to ChatGPT, Concerns from (1) academia and publishers. Policies w.r.t. ChatGPT-generate content; (2) content spam or fraud.
    \item However, the task of ChatGPT detection is not easy (the main obstacle in enforcing the policies). Reason is that the human-like style with word diversity makes the watermark (artifact) very subtle. Many existing detectors ({\newc please add examples}) may work well for earlier models ({\newc please add examples}) but fail ChatGPT detection.
    \item Although people have accumulated a variety of experiences in identifying ChatGPT text, human beings actually do very poorly. There comes the question: if we want to design a detector for ChatGPT, what information/feature will work? There is a lack of systematic studies to address this question.
    \item our study, (1) how to generate ChatGPT-vs-control samples in academic writing to conduct the investigation.
    \item (2) how to recruit humans for the identification test. How to design the questionnaire. Why a model-based approach is the solution.
    \item (3) how to develop a model-based detection model. To validate the effectiveness, how to design the evaluation: cross-task, transfer learning. How to interpret the result to verify our conclusion: a watermark (signature) in chatGPT can be effectively captured in the senescence level.
\end{itemize}
\fi

==> CheckGPT/tex/related.tex <==
\section{Related Work}\label{sec:related}
\noindent\textbf{Neural Language Model.} The neural networks for word probability modeling have been developed since the 2000s \cite{bengio2000neural, sundermeyer2012lstm, cho2014learning}. Recently, pre-trained language models have been widely used because of the general but effective word representation, e.g., BERT \cite{devlin2018bert}, RoBERTa \cite{liu2019roberta}, ELMo \cite{emlo2018}, GPT-2 \cite{radford2019language}, and BART \cite{lewis2019bart}. 


\noindent\textbf{LLM-Content Generation and Detection.} Prior works \cite{gehrmann2019gltr, kushnareva2021artificial, mitchell2023detectgpt, theocharopoulos2023detection, zellers2019defending} study LLM-content detection for models before ChatGPT, e.g., Grover, GPT-2, and GPT-3. Recently, \cite{gao2022comparing} evaluated 50 ChatGPT-written biomedical research abstracts with human reviewers and a RoBERTa-based classifier. Their findings show that 34\% of the abstracts received scores <50\% from the classifier, i.e., they are labeled as likely human-written, while four human reviewers correctly identified 68\% of the GPT-written abstracts. \cite{bleuminkkeeping} trained a transformer-based deep learning model to distinguish between AI-generated and human-written essays in a range of different education levels. \cite{guo2023close} and \cite{liu2023argugpt} conduct comprehensive studies, including human evaluators. \cite{guo2023close} analyzes a series of question-answering datasets in both English and Chinese, and \cite{liu2023argugpt} targets the essays written by students and English learners. \cite{he2023mgtbench} establishes the first machine-generated text benchmark evaluating a number of detection approaches. The detailed comparisons of current GPT detectors are listed in Table~\ref{tab:literature}. Compared with the other approaches, \checkgpt~(1) collects and uses a significantly larger dataset, (2) uses a model-agnostic design for higher
affordability, upgradability, and flexibility, and (3) achieves very high accuracy, transferability, and interpretability. 

%Most of the other methods use smaller datasets, except \cite{guo2023close}, which 

\begin{table*}[ht!]
    \centering
    \caption{Summary of SOTA LLM-content Detectors. Tool: used/evaluated online detection tools. Open: open-sourced.}
    \vspace{-2mm}
    \label{tab:literature}
    \begin{footnotesize}
    \setlength{\tabcolsep}{0.7em}
    \begin{tabular}{|M{1.05cm}|M{0.6cm}||M{0.55cm}|M{0.8cm}|M{0.7cm}|M{0.85cm}||M{0.8cm}||M{1.2cm}||M{0.55cm}|M{0.55cm}|M{0.55cm}|M{1.0cm}||M{1cm}|M{0.55cm}|}
        \hline
        \multicolumn{2}{|c||}{\multirow{2}{*}{Study}} & \multicolumn{4}{c||}{Approach} &  \multirow{2}{*}{\parbox{0.8cm}{Transfer\\-ability}} & \# Human & \multicolumn{4}{c||}{Domain}  &  \multicolumn{2}{c|}{Dataset}   \\
        \cline{3-6}\cline{9-14}
         \multicolumn{2}{|c||}{}& Tool & Stat & Human & Train DNNs &&  Evaluators & News & QA & Essay & Research & Size & Open\\
        \hline
        
        \hline
         \multirow{5}{*}{\parbox{1.2cm}{Grover or\\GPT-2\&3}} 
        & \cite{gehrmann2019gltr} &
          & \ding{108}& &            &
          $-$ & $-$ & 
          \ding{108}& & & \ding{108}           & 
          $300$ &\\ 
         \cline{2-14}
         & \cite{kushnareva2021artificial} &
          & \ding{108}& &  \ding{108}          &
           $-$ & $-$ &
          \ding{108}& & &            & 
          $90k$ & \ding{108}\\ 
          \cline{2-14}
       
        & \cite{mitchell2023detectgpt} &
          \ding{108}& & &            &
           $-$ & $-$ &
          \ding{108} & & \ding{108} &            & 
          $-$ &\\
          \cline{2-14}
           & \cite{theocharopoulos2023detection} &
          & \ding{108}& & \ding{108}           &
           & $-$ &
          & & & \ding{108}           & 
          $28k$ & \ding{108} \\
        \cline{2-14}
         & \cite{zellers2019defending} &
          & & \ding{108} &  \ding{108}          &
           &  $*$ &
          \ding{108} & & &            & 
          $20k$ & \ding{108} \\ 
         \hline
         
         \hline
         
         \multirow{5}{*}{ChatGPT} 
            & \cite{bleuminkkeeping} &
          & & & \ding{108}           &
          & $-$ &
          & & \ding{108} &            & 
          $100k$&\\
         \cline{2-14}
         & \cite{gao2022comparing} &
          \ding{108}& & \ding{108}&            &
          $-$ & $2$ &
          & & &  \ding{108}          & 
          $100$&\\ 
        \cline{2-14}
        & \cite{guo2023close} &
          & \ding{108}& \ding{108}&  \ding{108}          &
          & $17$ &
          & \ding{108} & &            & 
          $125k$&\ding{108}\\
          \cline{2-14}
        % & \cite{he2023mgtbench} &
        %   \ding{108}& \ding{108}& & \ding{108}           &
        %   & \ding{108} & &            & 
        %   $2817$\\
        %  \cline{2-11}
        
        & \cite{he2023mgtbench} &
          \ding{108}& \ding{108}& & \ding{108}           & \ding{108}
          & &
          & \ding{108} & &            & 
          $6k$&\ding{108}\\
         \cline{2-14}
         
         & \cite{liu2023argugpt} &
          \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
          & $43$ &
          & & \ding{108} &            & 
          $8k$&\ding{108}\\
         \cline{2-14}

         & \cite{macko2023multitude} &
          \ding{108}& \ding{108}& & \ding{108}           &
          & &
         \ding{108} & &  &            & 
          $74k$&\ding{108}\\
         \cline{2-14}

         & \cite{wang2023m4} &
          & \ding{108}& & \ding{108}           &
          \ding{108} &  &
          \ding{108} & \ding{108} & \ding{108} &     \ding{108}       & 
          $122k$&\ding{108}\\
         \cline{2-14}

         & \cite{kumari2023demasq} &
          \ding{108} & \ding{108}& &            &
           &  &
           & \ding{108} &  &     \ding{108}       & 
          $134k$& \\
         \cline{2-14}
         
         & Ours &
          \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
          \ding{108} & {\color{blue}{\textbf{155 + 87}}} &
          \ding{108} & & \ding{108} &  \ding{108}          & 
          {\color{blue}{\textbf{>2385k}}}&\ding{108}\\
         \cline{2-14}
         \hline

         \hline
    \end{tabular}\\
\vspace{-3mm}
\begin{flushleft}
$*$ The number of human evaluators is not explicitly provided.
\end{flushleft}
\vspace{-4mm}
\end{footnotesize}
\end{table*}

\noindent\textbf{Security and Ethics in AIGC Application.} AI-generated content (AIGC) has been used in adversarial activities even before LLMs were introduced \cite{ferrara2016rise}, while the recent release of ChatGPT may have provided the malicious actors with a powerful tool \cite{renaud2023chatgpt,derner2023beyond}. In particular, the detection of AI-backed social bots, spam, scams, and misinformation has been extensively studied in the literature, e.g., \cite{cresci2020decade,shahid2022detecting,yang2020scalable,lu2022effects}, while the rise of LLMs and ChatGPT introduces both new opportunities \cite{heidari2021bert,heidari2020using,dukic2020you,garcia2019empirical,hoes2023using,wang2023bot} and challenges \cite{gradonm2023electric,de2023chatgpt,mansfield2023weaponising}. For instance, ChatGPT may be used in scamming or phishing \cite{grbic2023social,roy2023generating,hazell2023large} as well as in the defense \cite{cambiaso2023scamming}. While Open AI has enforced internal mechanisms to prohibit the unethical use of ChatGPT, the restrictions could be evaded through prompt engineering (jailbreaking) \cite{li2023multi,liu2023jailbreaking}. Finally, there are also discussions and concerns with ChatGPT's potential impact on education and research \cite{stokel2022ai,willems2023chatgpt, firat2023chatgpt}, especially on authorship and plagiarism  \cite{stokelchatgpt,flanagin2023nonhuman,khalil2023will,anders2023using}.  A small-scale experiment in \cite{gao2022comparing} showed that most of the GPT-generated abstracts were deemed as completely original by a web-based plagiarism detector (\url{https://plagiarismdetector.net/}).


==> CheckGPT/tex/survey.tex <==
\section{User Study: Identification of Human- and GPT-Generated Abstracts}\label{sec:survey}

With all the news reports and online/informal discussions that human users are unable to distinguish ChatGPT-generated text from man-written text, we investigate this problem through a user study in a relatively well-defined domain: research publications. We aim to answer four research questions: 

\vspace{3pt}
\noindent
\textbf{RQ1:} Could (experienced) researchers distinguish between human-written and GPT-generated paper abstracts?

\vspace{3pt}
\noindent
\textbf{RQ2:} Do prior experiences with reading/writing papers contribute to the capability of identifying GPT-generated abstracts? 

\vspace{3pt}
\noindent
\textbf{RQ3:} Does the researchers' capability in identifying GPT content 
vary by discipline? 

\vspace{3pt}
\noindent
\textbf{RQ4:} Will their capability improve if they have ground truth data (pairs of human- and GPT-generated content) as references?
\vspace{3pt}

We designed a questionnaire as follows: %\footnote{This user study was reviewed and approved by the Human Research Protection Program at [Anonymized] University.}: 
first, the landing page displays an IRB information statement and asks the participants to select their ``most familiar discipline'' among CS, Physics, and Humanities \& Social Sciences (HSS). Then, the main questionnaire page asks the participants to provide basic background information, their roles, whether they have published research papers, and self-claimed familiarity with research papers. Finally, each participant is presented with three abstracts and asked to annotate each as ``human-written'' or ``GPT-GEN/POL''. Each abstract is randomly sampled from HUM or GPT-WRI/POL abstracts from Tasks 1 and 3 of GPABench2. For Task 3, we display the following hint: ``This abstract was completely written by humans OR written by humans and then polished by ChatGPT.'' 

In the second experiment, we provide the participant with some ground truth data as reference, i.e., we display three pairs of labeled human- and GPT-generated abstracts from the same task and the same discipline, and instruct the participants to learn the writing styles from these abstracts before moving to the detection questions. Three unlabeled samples are then displayed to the user to annotate. 

\begin{table}[t]
	\caption{Results of the user study. Par.: number of participants; Acc.: accuracy; HUM: accuracy for human-written abstracts; GPT: accuracy for GPT-generated abstracts.}\label{tab:userstudy1}
 \vspace{-4mm}
    \setlength{\tabcolsep}{2pt}
    \centering
    {
	\begin{tabular}{c|cccc|cccc}
        \hline
        & \multicolumn{4}{c|}{Exp 1: w/o reference} & \multicolumn{4}{c}{Exp 2: with reference} \\ \hline
	      Category & Par. & Acc. & HUM & GPT  & Par. & Acc. & HUM & GPT \\\hline
        \multicolumn{9}{c}{Role}\\\hline
Faculty & 	44 & 49.2\% & 	58.6\% & 	41.9\%  & 28 & 59.5\% & 61.2\% & 57.1\% \\
Researchers & 30 & 50.0\% & 	58.2\% & 	37.1\% & 28 & 58.3\% & 	56.3\% & 	61.1\% \\
Students & 	81 & 48.1\% & 	56.3\% & 	40.3\%  & 31 & 66.7\% & 	75.6\% & 	58.3\% \\ 
        \hline
        \multicolumn{9}{c}{Discipline}\\\hline
CS & 	57 & 50.3\% & 	59.0\% & 	43.0\% & 33 & 60.6\% & 	59.6\% & 61.5\%\\
Physics & 	48 &	53.5\% & 	65.1\% & 37.7\% & 25 & 60.0\% & 	71.1\% & 	43.3\%\\
HSS & 	50 & 42.7\% & 	46.5\% & 	39.2\% & 29 & 64.4\% & 	62.0\% & 	67.6\% \\
        \hline
        \multicolumn{9}{c}{Self-claimed Familiarity with Research Papers}\\\hline
Expert & 	52  & 	51.3\% & 	60.6\% & 	43.5\%  & 32 & 61.5\% & 	67.3\% & 	53.7\% \\
Knowledgable & 	56 & 	47.6\% & 	57.3\% & 	34.7\% & 30 & 61.1\% & 	56.5\% & 	65.9\% \\
Somewhat & 	39 & 48.7\% & 	56.0\% & 	43.3\% & 21 & 65.1\% & 	72.7\% & 56.7\% \\
No familiarity & 8  & 	41.7\% & 	46.7\% & 	33.3\% & 4 & 50.0\% & 	50.0\% & 	50.0\% \\
        \hline
        \multicolumn{9}{c}{Published papers?}\\\hline
Yes & 	106 & 48.7\% & 	58.1\% & 	39.2\% & 56 & 60.7\% & 	64.0\% & 	57.0\% \\
No & 	49 & 49.0\% & 	55.6\% & 	42.7\% & 31 & 63.4\% & 	64.2\% & 	62.5\% \\
        \hline
        \end{tabular}} \vspace{-4mm}
\end{table}

% \begin{table}[t]
% 	\caption{Results of the user study without examples. Par.: number of participants; Abs.: number of annotated abstracts; Cor.: number of correct annotations; Acc.: accuracy; HUM: accuracy for human-written abstracts; GPT: accuracy for GPT-generated abstracts.}\label{tab:userstudy1}
%  \vspace{-2mm}
%     \setlength{\tabcolsep}{1pt}
%     \centering
%     {
% 	\begin{tabular}{ccccccc}
% 		\hline
% 	      Category & Par. & Cor. & Acc. & HUM & GPT \\\hline
%         \multicolumn{7}{c}{Role}\\\hline
% Faculty & 	44 & 132 & 	65 & 	49.2\% & 	58.6\% & 	41.9\% \\
% Researchers & 	30 & 90 & 	45 & 	50.0\% & 	58.2\% & 	37.1\% \\
% Students & 	81 & 243 & 	117 & 	48.1\% & 	56.3\% & 	40.3\% \\ 
%         \hline
%         \multicolumn{7}{c}{Discipline}\\\hline
% CS & 	57 & 171 & 	86 & 	50.3\% & 	59.0\% & 	43.0\% \\
% Physics & 	48 & 144 & 	77 & 	53.5\% & 	65.1\% & 	37.7\% \\
% HSS & 	50 & 150 & 	64 & 	42.7\% & 	46.5\% & 	39.2\% \\
%         \hline
%         \multicolumn{7}{c}{Self-claimed Familiarity with Research Papers}\\\hline
% Expert & 	52 & 156 & 	80 & 	51.3\% & 	60.6\% & 	43.5\% \\
% Knowledgable & 	56 & 168 & 	80 & 	47.6\% & 	57.3\% & 	34.7\% \\
% Somewhat & 	39 & 117 & 	57 & 	48.7\% & 	56.0\% & 	43.3\% \\
% No familiarity & 	8 & 24 & 	10 & 	41.7\% & 	46.7\% & 	33.3\% \\
%         \hline
%         \multicolumn{7}{c}{Published papers?}\\\hline
% Yes & 	106 & 318 & 	155 & 	48.7\% & 	58.1\% & 	39.2\% \\
% No & 	49 & 147 & 	72 & 	49.0\% & 	55.6\% & 	42.7\% \\
%         \hline
%         \end{tabular}} \vspace{-4mm}
% \end{table}


% \begin{table}[t]
% {\newc 
% 	\caption{Results of the user study with examples provided.}\label{tab:userstudy2}
%  \vspace{-2mm}
%     \setlength{\tabcolsep}{0.5em}
%     \centering
%     {
% 	\begin{tabular}{ccccccc}
% 		\hline
% 	      Category & Par. & Abs. & Cor. & Acc. & HUM & GPT \\\hline
%         \multicolumn{7}{c}{Role}\\\hline
% Faculty & 28 & 84 & 50 & 59.5\% & 	61.2\% & 57.1\% \\
% Researchers & 28 & 84 & 49 & 58.3\% & 	56.3\% & 61.1\% \\
% Students & 31 & 93 & 62 & 66.7\% & 75.6\%	& 58.3\%	 \\ 
%         \hline
%         \multicolumn{7}{c}{Discipline}\\\hline
% CS & 33 & 99 & 60 & 60.6\% & 59.6\% & 61.5\% \\
% Physics & 25 & 75 & 45 & 60.0\% & 71.1\%	 & 	43.3\% \\
% HSS & 29 & 87 & 56 & 64.4\% & 62.0\% & 67.6\%\\
%         \hline
%         \multicolumn{7}{c}{Self-claimed Familiarity with Research Papers}\\\hline
% Expert & 32	& 96 & 59	 & 	61.5\% & 	67.3\% & 53.7\%	 \\
% Knowledgable & 30	& 90 & 	55 & 	61.1\% & 	56.5\% & 	65.9\% \\
% Somewhat & 21	& 63 & 	27 & 64.3\%	 & 	72.7\% & 56.7\%	 \\
% No familiarity & 4	& 12 & 	6 & 50.0\%	 & 50.0\%	 & 	50.0\% \\
%         \hline
%         \multicolumn{7}{c}{Published papers?}\\\hline
% Yes & 56	& 168 & 102	 & 60.7\%	 & 64.0\%	 & 57.0\%	 \\
% No & 31	& 93 & 59 & 	63.4\% & 64.2\%	 & 62.5\%	 \\
%         \hline
%         \end{tabular}} \vspace{-4mm}
%         }
% \end{table}


% We distributed questionnaires to faculty members, researchers, and graduate students in the Departments of EECS, Physics, and College of Liberal Arts at our University (in the US) and %Physics faculty members disseminated the questionnaires to  collaborators in 
% a research organization in Europe. 
% In four weeks, we received 155 responses with 465 annotated abstracts. The overall accuracy was 48.82\%, which is slightly worse than random guesses. The detailed statistics are shown in Table~\ref{tab:userstudy}. From the responses, we have the following observations: (1) It is very challenging for human users to distinguish between human-written and GPT-generated paper abstracts (only 21 users correctly identified all three abstracts). (2) Participants have the tendency to annotate  abstracts as ``human-written'', i.e., 59.66\% of GPT-generated abstracts were mistakenly labeled as ``human''. The results confirm the public opinion that ChatGPT achieves human-like language style and quality. (3) Users perform better in identifying GPT-written abstracts and worse in GPT-polished abstracts. (4) Users' self-claimed expertise only slightly affects their identification capability. And (5) users perform better in physics and significantly worse in humanity and social sciences. 

We distributed questionnaires to faculty members, researchers, and graduate students in the Department of EECS, Department of Physics, and College of Liberal Arts at our University (in the US). Physics faculty members also shared the questionnaire with collaborators in a large research organization in Europe. For Experiment 1, we received 155 responses with 465 annotated abstracts in approximately four weeks. The overall accuracy, defined as the proportion of correctly identified abstracts out of all abstracts, was 48.82\%, which is slightly worse than random guesses. For Experiment 2, we received 87 responses with 261 annotated abstracts in two weeks. The overall accuracy improved to 61.69\%. Note that the median time spent on each questionnaire was 108 seconds in Experiment 1 and 229 seconds in Experiment 2, showing that the participants did spend time reading and comprehending the ground truth samples. The detailed statistics of the responses are shown in Table~\ref{tab:userstudy1}. From the responses, we have the following observations:

\noindent$\bullet~$ It is very challenging for human users to distinguish between human-written and GPT-generated paper abstracts. Only 21 users in Experiment 1 and 24 users in Experiment 2 correctly identified all three abstracts. If all participants were making random selections, 19.38 users would have scored 3 correct selections in Experiment 1. %That is, the top performers are only slightly better than random guesses. 

\noindent$\bullet~$ Participants have the tendency to annotate abstracts as ``human''. 57.33\% and 64.08\% of human-written abstracts were correctly labeled as ``human-written" in Experiments 1 and 2, respectively, while 59.66\% and 41.2\% of GPT-generated abstracts were mistakenly labeled as ``human-written''. The result confirms the public opinion that ChatGPT achieves human-like language style and quality. 

\noindent$\bullet~$Users are better at identifying fully GPT-written abstracts with the accuracy of 43.81\% and 66.13\%, while they perform worse with GPT-polished abstracts with the accuracy of 37.5\% and 50.88\%. %In both cases, the accuracy is still lower than random guesses. 

\noindent$\bullet~$ Users' self-claimed expertise appears to very slightly affect their capability to identify human-written and GPT-generated abstracts. For example, participants with ``No familiarity'' with papers performed worse than the others. However, most of the differences are \textit{not} statistically significant. 
    
\noindent$\bullet~$ Users become slightly better at identifying GPT-generated content when they are provided with references. However, the accuracy is still too low for reliable identification. The largest improvement is witnessed in HSS with an accuracy improvement of 21.5\%.

% \begin{itemize}[noitemsep, topsep=1mm, left=0pt]
%     \item It is extremely challenging for human users to distinguish between human-written and GPT-generated paper abstracts. Only 21 users correctly identified all three abstracts. If all participants were making random selections, 19.38 users would have scored 3 correct selections. That is, the top performers are only slightly better than random guesses. 
%     \item Participants have the tendency to annotate all abstracts as ``human-written''. 57.33\% of human-written abstracts were correctly labeled as ``human-written", while 59.66\% of GPT-generated abstracts were mistakenly labeled as ``human-written''. The result confirms the public opinion that ChatGPT achieves human-like language style and quality. 
%     \item Users are better at identifying fully GPT-written abstracts with an accuracy of 43.81\%, while they perform worse with GPT-polished abstracts with an accuracy of 37.5\%. In both cases, the accuracy is still lower than random guesses. 
%     \item Users' self-claimed expertise appears to slightly affect their capability to identify human-written and GPT-generated abstracts. For example, participants with ``No familiarity'' with papers performed worse than the others. However, most of the differences are \textit{not} statistically significant. 
%     \item Users are better at identifying GPT-generated abstracts in physics. They are significantly worse at identifying GPT-generated abstracts in humanity and social sciences. 
%     \item {\newc Users become slightly better at identifying GPT-generated abstracts. However, the accuracy is still too low for reliable identification. The largest improvement is witnessed in HSS with an increased accuracy of 21.5\%.}
% \end{itemize}





==> tex/related.tex <==
\section{Related Work}\label{sec:related}
\noindent\textbf{Neural Language Model.} The neural networks for word probability modeling have been developed since the 2000s \cite{bengio2000neural, sundermeyer2012lstm, cho2014learning}. Recently, pre-trained language models have been widely used because of the general but effective word representation, e.g., BERT \cite{devlin2018bert}, RoBERTa \cite{liu2019roberta}, ELMo \cite{emlo2018}, GPT-2 \cite{radford2019language}, and BART \cite{lewis2019bart}. 


\noindent\textbf{LLM-Content Generation and Detection.} Prior works \cite{gehrmann2019gltr, kushnareva2021artificial, mitchell2023detectgpt, theocharopoulos2023detection, zellers2019defending} study LLM-content detection for models before ChatGPT, e.g., Grover, GPT-2, and GPT-3. Recently, \cite{gao2022comparing} evaluated 50 ChatGPT-written biomedical research abstracts with human reviewers and a RoBERTa-based classifier. Their findings show that 34\% of the abstracts received scores <50\% from the classifier, i.e., they are labeled as likely human-written, while four human reviewers correctly identified 68\% of the GPT-written abstracts. \cite{bleuminkkeeping} trained a transformer-based deep learning model to distinguish between AI-generated and human-written essays in a range of different education levels. \cite{guo2023close} and \cite{liu2023argugpt} conduct comprehensive studies, including human evaluators. \cite{guo2023close} analyzes a series of question-answering datasets in both English and Chinese, and \cite{liu2023argugpt} targets the essays written by students and English learners. \cite{he2023mgtbench} establishes the first machine-generated text benchmark evaluating a number of detection approaches. The detailed comparisons of current GPT detectors are listed in Table~\ref{tab:literature}. Compared with the other approaches, \checkgpt~(1) collects and uses a significantly larger dataset, (2) uses a model-agnostic design for higher
affordability, upgradability, and flexibility, and (3) achieves very high accuracy, transferability, and interpretability. 

%Most of the other methods use smaller datasets, except \cite{guo2023close}, which 

\begin{table*}[ht!]
    \centering
    \caption{Summary of SOTA LLM-content Detectors. Tool: used/evaluated online detection tools. Open: open-sourced.}
    \vspace{-2mm}
    \label{tab:literature}
    \begin{footnotesize}
    \setlength{\tabcolsep}{0.7em}
    \begin{tabular}{|M{1.05cm}|M{0.6cm}||M{0.55cm}|M{0.8cm}|M{0.7cm}|M{0.85cm}||M{0.8cm}||M{1.2cm}||M{0.55cm}|M{0.55cm}|M{0.55cm}|M{1.0cm}||M{1cm}|M{0.55cm}|}
        \hline
        \multicolumn{2}{|c||}{\multirow{2}{*}{Study}} & \multicolumn{4}{c||}{Approach} &  \multirow{2}{*}{\parbox{0.8cm}{Transfer\\-ability}} & \# Human & \multicolumn{4}{c||}{Domain}  &  \multicolumn{2}{c|}{Dataset}   \\
        \cline{3-6}\cline{9-14}
         \multicolumn{2}{|c||}{}& Tool & Stat & Human & Train DNNs &&  Evaluators & News & QA & Essay & Research & Size & Open\\
        \hline
        
        \hline
         \multirow{5}{*}{\parbox{1.2cm}{Grover or\\GPT-2\&3}} 
        & \cite{gehrmann2019gltr} &
          & \ding{108}& &            &
          $-$ & $-$ & 
          \ding{108}& & & \ding{108}           & 
          $300$ &\\ 
         \cline{2-14}
         & \cite{kushnareva2021artificial} &
          & \ding{108}& &  \ding{108}          &
           $-$ & $-$ &
          \ding{108}& & &            & 
          $90k$ & \ding{108}\\ 
          \cline{2-14}
       
        & \cite{mitchell2023detectgpt} &
          \ding{108}& & &            &
           $-$ & $-$ &
          \ding{108} & & \ding{108} &            & 
          $-$ &\\
          \cline{2-14}
           & \cite{theocharopoulos2023detection} &
          & \ding{108}& & \ding{108}           &
           & $-$ &
          & & & \ding{108}           & 
          $28k$ & \ding{108} \\
        \cline{2-14}
         & \cite{zellers2019defending} &
          & & \ding{108} &  \ding{108}          &
           &  $*$ &
          \ding{108} & & &            & 
          $20k$ & \ding{108} \\ 
         \hline
         
         \hline
         
         \multirow{5}{*}{ChatGPT} 
            & \cite{bleuminkkeeping} &
          & & & \ding{108}           &
          & $-$ &
          & & \ding{108} &            & 
          $100k$&\\
         \cline{2-14}
         & \cite{gao2022comparing} &
          \ding{108}& & \ding{108}&            &
          $-$ & $2$ &
          & & &  \ding{108}          & 
          $100$&\\ 
        \cline{2-14}
        & \cite{guo2023close} &
          & \ding{108}& \ding{108}&  \ding{108}          &
          & $17$ &
          & \ding{108} & &            & 
          $125k$&\ding{108}\\
          \cline{2-14}
        % & \cite{he2023mgtbench} &
        %   \ding{108}& \ding{108}& & \ding{108}           &
        %   & \ding{108} & &            & 
        %   $2817$\\
        %  \cline{2-11}
        
        & \cite{he2023mgtbench} &
          \ding{108}& \ding{108}& & \ding{108}           & \ding{108}
          & &
          & \ding{108} & &            & 
          $6k$&\ding{108}\\
         \cline{2-14}
         
         & \cite{liu2023argugpt} &
          \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
          & $43$ &
          & & \ding{108} &            & 
          $8k$&\ding{108}\\
         \cline{2-14}

         & \cite{macko2023multitude} &
          \ding{108}& \ding{108}& & \ding{108}           &
          & &
         \ding{108} & &  &            & 
          $74k$&\ding{108}\\
         \cline{2-14}

         & \cite{wang2023m4} &
          & \ding{108}& & \ding{108}           &
          \ding{108} &  &
          \ding{108} & \ding{108} & \ding{108} &     \ding{108}       & 
          $122k$&\ding{108}\\
         \cline{2-14}

         & \cite{kumari2023demasq} &
          \ding{108} & \ding{108}& &            &
           &  &
           & \ding{108} &  &     \ding{108}       & 
          $134k$& \\
         \cline{2-14}
         
         & Ours &
          \ding{108}& \ding{108}& \ding{108}& \ding{108}           &
          \ding{108} & {\color{blue}{\textbf{155 + 87}}} &
          \ding{108} & & \ding{108} &  \ding{108}          & 
          {\color{blue}{\textbf{>2385k}}}&\ding{108}\\
         \cline{2-14}
         \hline

         \hline
    \end{tabular}\\
\vspace{-3mm}
\begin{flushleft}
$*$ The number of human evaluators is not explicitly provided.
\end{flushleft}
\vspace{-4mm}
\end{footnotesize}
\end{table*}

\noindent\textbf{Security and Ethics in AIGC Application.} AI-generated content (AIGC) has been used in adversarial activities even before LLMs were introduced \cite{ferrara2016rise}, while the recent release of ChatGPT may have provided the malicious actors with a powerful tool \cite{renaud2023chatgpt,derner2023beyond}. In particular, the detection of AI-backed social bots, spam, scams, and misinformation has been extensively studied in the literature, e.g., \cite{cresci2020decade,shahid2022detecting,yang2020scalable,lu2022effects}, while the rise of LLMs and ChatGPT introduces both new opportunities \cite{heidari2021bert,heidari2020using,dukic2020you,garcia2019empirical,hoes2023using,wang2023bot} and challenges \cite{gradonm2023electric,de2023chatgpt,mansfield2023weaponising}. For instance, ChatGPT may be used in scamming or phishing \cite{grbic2023social,roy2023generating,hazell2023large} as well as in the defense \cite{cambiaso2023scamming}. While Open AI has enforced internal mechanisms to prohibit the unethical use of ChatGPT, the restrictions could be evaded through prompt engineering (jailbreaking) \cite{li2023multi,liu2023jailbreaking}. Finally, there are also discussions and concerns with ChatGPT's potential impact on education and research \cite{stokel2022ai,willems2023chatgpt, firat2023chatgpt}, especially on authorship and plagiarism  \cite{stokelchatgpt,flanagin2023nonhuman,khalil2023will,anders2023using}.  A small-scale experiment in \cite{gao2022comparing} showed that most of the GPT-generated abstracts were deemed as completely original by a web-based plagiarism detector (\url{https://plagiarismdetector.net/}).

